Algebraic Combinatorics of Magic Squares

We describe how to construct and enumerate Magic squares, Franklin squares, Magic cubes, and Magic graphs as lattice points inside polyhedral cones using techniques from Algebraic Combinatorics. The main tools of our methods are the Hilbert Poincare series to enumerate lattice points and the Hilbert bases to generate lattice points. We define polytopes of magic labelings of graphs and digraphs, and give a description of the faces of the Birkhoff polytope as polytopes of magic labelings of digraphs.

==> figures/3x3magichbasis <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 600 900 600 1800 1500 1800 1500 900 600 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 900 900 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 900 1200 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 1200 1500 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 1500 1500 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 2100 900 2100 1800 3000 1800 3000 900 2100 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 3600 900 3600 1800 4500 1800 4500 900 3600 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 5100 900 5100 1800 6000 1800 6000 900 5100 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 6600 900 6600 1800 7500 1800 7500 900 6600 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2100 1200 3000 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2100 1500 3000 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 1200 4500 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 1500 4500 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 1200 6000 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 1500 6000 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6600 1200 7500 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6600 1500 7500 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 900 2400 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 900 2700 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3900 900 3900 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4200 900 4200 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 900 5400 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5700 900 5700 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 900 6900 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 900 7200 1800
4 0 0 50 0 0 12 0.0000 4 135 720 675 1125  1     0    2\001
4 0 0 50 0 0 12 0.0000 4 135 720 675 1425 2      1    0\001
4 0 0 50 0 0 12 0.0000 4 135 720 675 1725 0     2     1\001
4 0 0 50 0 0 12 0.0000 4 135 720 2175 1125 2      0    1\001
4 0 0 50 0 0 12 0.0000 4 135 720 2175 1425 0      1    2\001
4 0 0 50 0 0 12 0.0000 4 135 720 2175 1725 1      2    0\001
4 0 0 50 0 0 12 0.0000 4 135 720 3675 1125  0    2     1\001
4 0 0 50 0 0 12 0.0000 4 135 720 3675 1425 2      1    0\001
4 0 0 50 0 0 12 0.0000 4 135 720 3675 1725 1      0    2\001
4 0 0 50 0 0 12 0.0000 4 135 720 5175 1125  1    2     0\001
4 0 0 50 0 0 12 0.0000 4 135 720 5175 1425 0     1     2\001
4 0 0 50 0 0 12 0.0000 4 135 720 5175 1725 2     0     1\001
4 0 0 50 0 0 12 0.0000 4 135 720 6675 1125  1     1    1\001
4 0 0 50 0 0 12 0.0000 4 135 720 6675 1425  1     1    1\001
4 0 0 50 0 0 12 0.0000 4 135 720 6675 1725  1     1    1\001


==> figures/4x4magichilbert <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 600 1200 600 2400 1800 2400 1800 1200 600 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 2700 1200 2700 2400 3900 2400 3900 1200 2700 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 4800 1200 4800 2400 6000 2400 6000 1200 4800 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 6900 1200 6900 2400 8100 2400 8100 1200 6900 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 9000 1200 9000 2400 10200 2400 10200 1200 9000 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 600 3300 600 4500 1800 4500 1800 3300 600 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 2700 3300 2700 4500 3900 4500 3900 3300 2700 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 4800 3300 4800 4500 6000 4500 6000 3300 4800 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 6900 3300 6900 4500 8100 4500 8100 3300 6900 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 9000 3300 9000 4500 10200 4500 10200 3300 9000 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 600 5400 600 6600 1800 6600 1800 5400 600 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 600 7500 600 8700 1800 8700 1800 7500 600 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 2700 5400 2700 6600 3900 6600 3900 5400 2700 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 4800 5400 4800 6600 6000 6600 6000 5400 4800 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 6900 5400 6900 6600 8100 6600 8100 5400 6900 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 9000 5400 9000 6600 10200 6600 10200 5400 9000 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 2700 7500 2700 8700 3900 8700 3900 7500 2700 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 4800 7500 4800 8700 6000 8700 6000 7500 4800 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 6900 7500 6900 8700 8100 8700 8100 7500 6900 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 9000 7500 9000 8700 10200 8700 10200 7500 9000 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 2400 900 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 1500 3900 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 1800 3900 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 2100 3900 2100
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 1500 6000 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 1800 6000 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 2100 6000 2100
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 1500 8100 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 1800 8100 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 2100 8100 2100
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 1500 10200 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 1800 10200 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 2100 10200 2100
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 3600 10200 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 3900 10200 3900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 4200 10200 4200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 5700 10200 5700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 6000 10200 6000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 6300 10200 6300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 7800 10200 7800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 8100 10200 8100
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 8400 10200 8400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 7800 8100 7800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 8100 8100 8100
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 8400 8100 8400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 7800 6000 7800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 8100 6000 8100
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 8400 6000 8400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 7800 3900 7800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 8100 3900 8100
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 8400 3900 8400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 7800 1800 7800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 8100 1800 8100
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 8400 1800 8400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 5700 1800 5700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 6000 1800 6000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 6300 1800 6300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 5700 3900 5700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 5700 3900 5700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 6000 3900 6000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 6300 3900 6300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 5700 6000 5700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 6000 6000 6000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 6300 6000 6300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 3600 8100 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 3900 8100 3900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 4200 8100 4200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 3600 6000 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 3900 6000 3900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 4200 6000 4200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 5700 8100 5700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 6000 8100 6000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 6300 8100 6300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 3600 3900 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 3900 3900 3900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 4200 3900 4200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 3600 1800 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 3900 1800 3900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 4200 1800 4200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 1500 1800 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 1800 1800 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 2100 1800 2100
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 2400 1200 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1500 2400 1500 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 2400 3000 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 2400 3300 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 2400 3600 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 2400 5100 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 2400 5400 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5700 2400 5700 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 2400 7200 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7500 2400 7500 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 2400 7800 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9300 2400 9300 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9600 2400 9600 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9900 2400 9900 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9300 4500 9300 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9900 4500 9900 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9600 4500 9600 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9300 6600 9300 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9600 6600 9600 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9900 6600 9900 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 4500 7800 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7500 4500 7500 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 4500 7200 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5700 4500 5700 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 4500 5400 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 4500 5100 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 4500 3600 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 4500 3300 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 4500 3000 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1500 4500 1500 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 4500 1200 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 4500 900 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 6600 900 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 6600 1200 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1500 6600 1500 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 6600 3000 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 6600 3300 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 6600 3600 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 6600 5100 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 6600 5400 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5700 6600 5700 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 8700 900 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 8700 1200 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1500 8700 1500 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 8700 3000 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 8700 3300 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 8700 3600 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 8700 5100 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 8700 5400 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5700 8700 5700 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 8700 7200 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 8700 7200 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9300 8700 9300 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9300 8700 9300 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9600 8700 9600 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9600 8700 9600 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9900 8700 9900 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 6600 7200 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7500 6600 7500 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 6600 7800 5400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7500 8700 7500 7500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 8700 7800 7500
4 0 0 50 0 0 12 0.0000 4 135 1035 675 1425 0      0     1    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 675 1725 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 675 2025 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 675 2325 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2775 1425 0      0     1    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2775 1725 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2775 2025 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2775 2325 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 4875 1425 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 6975 1725 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 4875 1725 0      0     1    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 6975 2025 0      0     1    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 4875 2325 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 6975 2325 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 4875 2025 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 6975 1425 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 9075 1425 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 675 4125 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2775 3825 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 4875 3525 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 9075 1725 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 675 3825 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2775 3525 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 4875 4425 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 9075 2325 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 675 3525 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2775 4125 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 4875 4125 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 9075 2025 0      0     1    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 675 4425 0      0     1    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2775 4425 0      0     1    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 4875 3825 0      0     1    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 675 5625 1     0     1     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 675 5925 0      0     0    2\001
4 0 0 50 0 0 12 0.0000 4 135 1035 675 6225 0     1     1     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 675 6525 1      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2775 5625  0     0    2     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2775 5925 0      1    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2775 6225 1      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2775 6525 1      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 4875 5625  0     0    1     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 4875 5925 0      1     0    1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 4875 6225 1      0     1    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 4875 6525 1      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 6975 5625 1      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 6975 5925 0     1     1     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 6975 6225 0      0     0    2\001
4 0 0 50 0 0 12 0.0000 4 135 1035 6975 6525 1      0     1    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 6975 3525 1      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 6975 3825 1      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 6975 4125 0      1    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 6975 4425 0      0     2    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 9075 3525 0      1    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 9075 3825 1      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1260 9075 4125 0      0     1    1     \001
4 0 0 50 0 0 12 0.0000 4 135 1035 9075 4425 1     0      1    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 9075 5625 1      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1260 9075 5925 0      0     1    1     \001
4 0 0 50 0 0 12 0.0000 4 135 1035 9075 6525 0      2     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 9075 6225 1      0     1    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 675 7725 0      2     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 675 8025 1      0     1    0\001
4 0 0 50 0 0 12 0.0000 4 135 1260 675 8325 0      0     1    1     \001
4 0 0 50 0 0 12 0.0000 4 135 1035 675 8625 1      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2775 7725 1      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2775 8025 1      0     1    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2775 8325 0      1     0    1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2775 8625 0      0     1    1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 4875 7725 0      1     0    1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 4875 8325 0     1     1     0\001
4 0 0 50 0 0 12 0.0000 4 135 1260 4875 8625 0      0     1    1     \001
4 0 0 50 0 0 12 0.0000 4 135 990 4875 8025 2      0    0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 6975 7725 1      0     1    0\001
4 0 0 50 0 0 12 0.0000 4 135 1260 6975 8025 0      0     1    1     \001
4 0 0 50 0 0 12 0.0000 4 135 1035 6975 8325 1      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 6975 8625 0      1     0    1\001
4 0 0 50 0 0 12 0.0000 4 135 1260 9075 7725 0      0     1    1     \001
4 0 0 50 0 0 12 0.0000 4 135 1035 9075 8025 0     1     1     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 9075 8325 2      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 9075 8625 0      1     0    1\001
4 0 0 50 0 0 12 0.0000 4 135 180 1125 2775 h1\001
4 0 0 50 0 0 12 0.0000 4 135 270 5325 6975 h13\001
4 0 0 50 0 0 12 0.0000 4 135 180 3225 2775 h2\001
4 0 0 50 0 0 12 0.0000 4 135 180 5325 2775 h3\001
4 0 0 50 0 0 12 0.0000 4 135 180 7425 2775 h4\001
4 0 0 50 0 0 12 0.0000 4 135 180 9525 2775 h5\001
4 0 0 50 0 0 12 0.0000 4 135 180 1125 4875 h6\001
4 0 0 50 0 0 12 0.0000 4 135 180 3225 4875 h7\001
4 0 0 50 0 0 12 0.0000 4 135 180 5325 4875 h8\001
4 0 0 50 0 0 12 0.0000 4 135 180 7425 4875 h9\001
4 0 0 50 0 0 12 0.0000 4 135 270 9525 4875 h10\001
4 0 0 50 0 0 12 0.0000 4 135 270 1125 6975 h11\001
4 0 0 50 0 0 12 0.0000 4 135 270 3225 6975 h12\001
4 0 0 50 0 0 12 0.0000 4 135 270 7350 6975 h14\001
4 0 0 50 0 0 12 0.0000 4 135 270 9450 6975 h15\001
4 0 0 50 0 0 12 0.0000 4 135 270 1125 9075 h16\001
4 0 0 50 0 0 12 0.0000 4 135 270 3225 9075 h17\001
4 0 0 50 0 0 12 0.0000 4 135 270 5325 9075 h18\001
4 0 0 50 0 0 12 0.0000 4 135 270 7425 9075 h19\001
4 0 0 50 0 0 12 0.0000 4 135 270 9525 9075 h20\001


==> figures/Jainaconstruct <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 900 600 900 1800 2100 1800 2100 600 900 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 3000 600 3000 1800 4200 1800 4200 600 3000 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 5100 600 5100 1800 6300 1800 6300 600 5100 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 7200 600 7200 1800 8400 1800 8400 600 7200 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 900 2700 900 3900 2100 3900 2100 2700 900 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 3000 2700 3000 3900 4200 3900 4200 2700 3000 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 5100 2700 5100 3900 6300 3900 6300 2700 5100 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 7200 2700 7200 3900 8400 3900 8400 2700 7200 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 1800 1200 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 900 2100 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 1200 2100 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 1500 2100 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 900 4200 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 1200 4200 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 1500 4200 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 900 6300 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 1200 6300 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 1500 6300 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 1200 8400 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 1500 8400 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 3000 8400 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 3300 8400 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 3600 8400 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 3000 6300 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 3300 6300 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 3600 6300 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 3000 4200 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 3300 4200 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 3600 4200 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 3000 2100 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 3300 2100 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 3600 2100 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 900 8400 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1500 1800 1500 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1800 1800 1800 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 1800 3300 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 1800 3600 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3900 1800 3900 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 1800 5400 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5700 1800 5700 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 1800 6000 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7500 1800 7500 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 1800 7800 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8100 1800 8100 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 3900 1200 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1500 3900 1500 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1800 3900 1800 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 3900 3300 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 3900 3600 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3900 3900 3900 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 3900 5400 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5700 3900 5700 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 3900 6000 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7500 3900 7500 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 3900 7800 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8100 3900 8100 2700
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 825 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1080 3075 1125 0      0    1     0 \001
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 1425 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 1725 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 7275 825 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 7275 1125 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1080 7275 1425 0      0    1     0 \001
4 0 0 50 0 0 12 0.0000 4 135 1035 7275 1725 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 975 2925 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 975 3225 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 975 3525 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1080 975 3825 0      0    1     0 \001
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 2925 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 3225 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 3525 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1080 3075 3825 0      0    1     0 \001
4 0 0 50 0 0 12 0.0000 4 135 1035 5175 2925 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1080 5175 3225 0      0    1     0 \001
4 0 0 50 0 0 12 0.0000 4 135 1035 5175 3525 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 5175 3825 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1125 7275 2925 7    12     1   14 \001
4 0 0 50 0 0 12 0.0000 4 135 1080 7275 3225 2    13    8    11\001
4 0 0 50 0 0 12 0.0000 4 135 1035 7275 3525 16   3    10    5\001
4 0 0 50 0 0 12 0.0000 4 135 1035 7275 3825  9     6   15    4\001
4 0 0 50 0 0 18 0.0000 4 45 150 6675 3375 =\001
4 0 0 50 0 0 20 0.0000 4 195 285 2325 1200 +4\001
4 0 0 50 0 0 20 0.0000 4 195 285 4500 1200 +2\001
4 0 0 50 0 0 20 0.0000 4 195 285 6675 1275 +8\001
4 0 0 50 0 0 20 0.0000 4 195 285 525 3375 +3\001
4 0 0 50 0 0 20 0.0000 4 195 420 2400 3300 +12\001
4 0 0 50 0 0 20 0.0000 4 195 285 4500 3300 +4\001
4 0 0 50 0 0 12 0.0000 4 135 990 975 825 0     0     1    0\001
4 0 0 50 0 0 12 0.0000 4 135 990 975 1125 0     1     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 975 1425 0     0     0     1\001
4 0 0 50 0 0 12 0.0000 4 135 990 975 1725 1     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 5175 825 0     0     0     1\001
4 0 0 50 0 0 12 0.0000 4 135 990 5175 1125 1     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 990 5175 1425 0     0     1    0\001
4 0 0 50 0 0 12 0.0000 4 135 990 5175 1725 0     1     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 180 1425 2175 h1\001
4 0 0 50 0 0 12 0.0000 4 135 180 3525 2175 h3\001
4 0 0 50 0 0 12 0.0000 4 135 180 5625 2175 h4\001
4 0 0 50 0 0 12 0.0000 4 135 180 7725 2175 h5\001
4 0 0 50 0 0 12 0.0000 4 135 180 1425 4275 h6\001
4 0 0 50 0 0 12 0.0000 4 135 180 3525 4275 h7\001
4 0 0 50 0 0 12 0.0000 4 135 180 5625 4275 h8\001
4 0 0 50 0 0 12 0.0000 4 180 1485 7125 4275 Jaina  magic square\001


==> figures/ancientmagicsquares <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 900 1200 900 2100 1800 2100 1800 1200 900 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 2100 1200 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 1500 1800 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 1800 1800 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1500 2100 1500 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 2400 1200 2400 2400 3600 2400 3600 1200 2400 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 2400 2700 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 2400 3000 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 2400 3300 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 1500 3600 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 1800 3600 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 2100 3600 2100
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 4200 1200 4200 2400 5400 2400 5400 1200 4200 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4500 2400 4500 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 2400 4800 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 2400 5100 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4200 2100 5400 2100
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4200 1800 5400 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4200 1500 5400 1500
4 0 0 50 0 0 12 0.0000 4 135 855 975 1425  4     9    2   \001
4 0 0 50 0 0 12 0.0000 4 135 765 975 1725 3     5      7\001
4 0 0 50 0 0 12 0.0000 4 135 765 975 2025 8      1     6\001
4 0 0 50 0 0 16 0.0000 4 150 165 1275 2400 A\001
4 0 0 50 0 0 12 0.0000 4 135 1080 2475 1425 7     12    1   14\001
4 0 0 50 0 0 12 0.0000 4 135 1080 2475 1725 2    13    8    11\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2475 2025 16    3   10    5\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2475 2325 9      6   15    4\001
4 0 0 50 0 0 16 0.0000 4 150 135 2925 2700 B\001
4 0 0 50 0 0 16 0.0000 4 150 150 4725 2700 C\001
4 0 0 50 0 0 12 0.0000 4 135 1170 4275 1425 16    3    2    13  \001
4 0 0 50 0 0 12 0.0000 4 135 1125 4275 1725 5     10   11   8  \001
4 0 0 50 0 0 12 0.0000 4 135 1080 4275 2025 9     6     7    12\001
4 0 0 50 0 0 12 0.0000 4 135 990 4275 2325 4    15   14   1\001


==> figures/anotherjainaconstruct <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 900 600 900 1800 2100 1800 2100 600 900 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 3000 600 3000 1800 4200 1800 4200 600 3000 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 5100 600 5100 1800 6300 1800 6300 600 5100 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 7200 600 7200 1800 8400 1800 8400 600 7200 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 900 2700 900 3900 2100 3900 2100 2700 900 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 3000 2700 3000 3900 4200 3900 4200 2700 3000 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 5100 2700 5100 3900 6300 3900 6300 2700 5100 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 7200 2700 7200 3900 8400 3900 8400 2700 7200 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 1800 1200 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 900 2100 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 1200 2100 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 1500 2100 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 900 4200 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 1200 4200 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 1500 4200 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 900 6300 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 1200 6300 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 1500 6300 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 1200 8400 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 1500 8400 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 3000 8400 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 3300 8400 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 3600 8400 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 3000 6300 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 3300 6300 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 3600 6300 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 3000 4200 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 3300 4200 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 3600 4200 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 3000 2100 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 3300 2100 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 3600 2100 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 900 8400 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1500 1800 1500 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1800 1800 1800 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 1800 3300 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 1800 3600 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3900 1800 3900 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 1800 5400 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5700 1800 5700 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 1800 6000 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7500 1800 7500 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 1800 7800 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8100 1800 8100 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 3900 1200 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1500 3900 1500 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1800 3900 1800 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 3900 3300 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 3900 3600 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3900 3900 3900 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 3900 5400 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5700 3900 5700 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 3900 6000 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7500 3900 7500 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 3900 7800 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8100 3900 8100 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 -1200 600 -1200 1800 0 1800 0 600 -1200 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 -1200 2700 -1200 3900 0 3900 0 2700 -1200 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -900 1800 -900 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -600 1800 -600 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -300 1800 -300 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1200 900 0 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1200 1200 0 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1200 1500 0 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1200 3000 0 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1200 3300 0 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1200 3600 0 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -900 3900 -900 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -600 3900 -600 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -300 3900 -300 2700
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 825 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1080 3075 1125 0      0    1     0 \001
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 1425 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 1725 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 7275 825 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 7275 1125 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1080 7275 1425 0      0    1     0 \001
4 0 0 50 0 0 12 0.0000 4 135 1035 7275 1725 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 975 2925 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 975 3225 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 975 3525 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1080 975 3825 0      0    1     0 \001
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 2925 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 3225 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 3525 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1080 3075 3825 0      0    1     0 \001
4 0 0 50 0 0 12 0.0000 4 135 1035 5175 2925 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1080 5175 3225 0      0    1     0 \001
4 0 0 50 0 0 12 0.0000 4 135 1035 5175 3525 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 5175 3825 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1125 7275 2925 7    12     1   14 \001
4 0 0 50 0 0 12 0.0000 4 135 1080 7275 3225 2    13    8    11\001
4 0 0 50 0 0 12 0.0000 4 135 1035 7275 3525 16   3    10    5\001
4 0 0 50 0 0 12 0.0000 4 135 1035 7275 3825  9     6   15    4\001
4 0 0 50 0 0 18 0.0000 4 45 150 6675 3375 =\001
4 0 0 50 0 0 12 0.0000 4 135 1125 -1200 825   1     1     0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 -1125 1125 0      1    1     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 -1125 1425 0      0    0     2\001
4 0 0 50 0 0 12 0.0000 4 135 990 -1125 1725 1      0    1    0\001
4 0 0 50 0 0 12 0.0000 4 135 990 975 825  1    0     0    1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 975 1125 0     0     1     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 975 1425 1     0     1     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 975 1725 0     2     0     0\001
4 0 0 50 0 0 12 0.0000 4 135 990 5175 825  1     1    0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 5175 1125 1     0     1     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 5175 1425 0      1    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 5175 1725 0      0    1     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 -1125 2925  0    0     1     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 -1125 3225 0     1     1     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 -1125 3525 2     0     0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 -1125 3825 0     1     0     1\001
4 0 0 50 0 0 20 0.0000 4 195 285 300 1275 +2\001
4 0 0 50 0 0 20 0.0000 4 135 150 2475 1275 +\001
4 0 0 50 0 0 20 0.0000 4 195 285 4500 1275 +2\001
4 0 0 50 0 0 20 0.0000 4 195 285 6600 1275 +8\001
4 0 0 50 0 0 20 0.0000 4 135 150 375 3375 +\001
4 0 0 50 0 0 20 0.0000 4 135 150 -1575 3375 +\001
4 0 0 50 0 0 20 0.0000 4 195 420 2325 3375 +11\001
4 0 0 50 0 0 20 0.0000 4 135 150 4575 3375 +\001
4 0 0 50 0 0 12 0.0000 4 135 180 3525 2175 h3\001
4 0 0 50 0 0 12 0.0000 4 135 270 1425 2175 h15\001
4 0 0 50 0 0 12 0.0000 4 135 270 5625 2175 h17\001
4 0 0 50 0 0 12 0.0000 4 135 180 7725 2175 h5\001
4 0 0 50 0 0 12 0.0000 4 135 180 1500 4275 h6\001
4 0 0 50 0 0 12 0.0000 4 135 180 3525 4275 h7\001
4 0 0 50 0 0 12 0.0000 4 135 180 5625 4275 h8\001
4 0 0 50 0 0 12 0.0000 4 180 1440 7125 4200 Jaina magic square\001
4 0 0 50 0 0 12 0.0000 4 135 270 -675 4200 h20\001
4 0 0 50 0 0 12 0.0000 4 135 270 -675 2100 h14\001


==> figures/b3 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 5100 2400 75 75 5100 2400 5100 2475
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 4800 3000 75 75 4800 3000 4800 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 5400 3000 75 75 5400 3000 5400 3075
2 1 1 3 0 7 50 0 -1 8.000 0 0 -1 0 0 5
	 4500 1800 4500 3600 5700 3600 5700 1800 4500 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 5175 2475 5400 2925
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 4783 2913 5083 2463
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 4875 3000 5325 3000
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 7350 3000 6750 3000
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 8625 2925 8100 2925
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 8100 3075 8700 3075
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 6525 2700 6525 3300 9225 3300 9225 2700 6525 2700
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 4800 3075 4650 3375 4950 3375 4800 3075
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 5400 3075 5250 3375 5550 3375 5400 3075
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 5100 2400 5250 2100 4950 2100 5100 2400
	 0.000 -1.000 -1.000 0.000
4 0 0 50 0 0 12 0.0000 4 45 105 7650 3075 =\001


==> figures/b32dimfaces <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 3000 2400 75 75 3000 2400 3000 2475
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 2700 3000 75 75 2700 3000 2700 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 3300 3000 75 75 3300 3000 3300 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 5100 2400 75 75 5100 2400 5100 2475
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 4800 3000 75 75 4800 3000 4800 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 5400 3000 75 75 5400 3000 5400 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 7200 2400 75 75 7200 2400 7200 2475
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 6900 3000 75 75 6900 3000 6900 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 7500 3000 75 75 7500 3000 7500 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 9300 2400 75 75 9300 2400 9300 2475
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 9600 3000 75 75 9600 3000 9600 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 9000 3000 75 75 9000 3000 9000 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 11400 2400 75 75 11400 2400 11400 2475
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 11100 3000 75 75 11100 3000 11100 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 11700 3000 75 75 11700 3000 11700 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 13500 2400 75 75 13500 2400 13500 2475
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 13200 3000 75 75 13200 3000 13200 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 13800 3000 75 75 13800 3000 13800 3075
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 7275 2475 7500 2925
2 1 1 3 0 7 50 0 -1 8.000 0 0 -1 0 0 5
	 2400 1800 2400 3600 3600 3600 3600 1800 2400 1800
2 1 1 3 0 7 50 0 -1 8.000 0 0 -1 0 0 5
	 4500 1800 4500 3600 5700 3600 5700 1800 4500 1800
2 1 1 3 0 7 50 0 -1 8.000 0 0 -1 0 0 5
	 6600 1800 6600 3600 7800 3600 7800 1800 6600 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 4875 3000 5325 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 3075 2475 3225 2925
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 2775 3000 3225 3000
2 1 1 3 0 7 50 0 -1 8.000 0 0 -1 0 0 5
	 8700 1800 8700 3600 9900 3600 9900 1800 8700 1800
2 1 1 3 0 7 50 0 -1 8.000 0 0 -1 0 0 5
	 10800 1800 10800 3600 12000 3600 12000 1800 10800 1800
2 1 1 3 0 7 50 0 -1 8.000 0 0 -1 0 0 5
	 12900 1800 12900 3600 14100 3600 14100 1800 12900 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 5400 2925 5175 2475
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 5025 2475 4800 2925
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 7425 3000 6975 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 9600 2925 9375 2475
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 6900 2925 7200 2475
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 9075 3000 9525 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 9000 2925 9225 2475
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 11175 3000 11625 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 11100 2925 11325 2475
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 11475 2475 11700 2925
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 9600 4500 9000 4500
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 10875 4500 10350 4500
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 10350 4650 10950 4650
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 8700 4200 8700 4800 11400 4800 11400 4200 8700 4200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 13245 2910 13470 2460
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 13575 2474 13725 2924
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 13275 3000 13725 3000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 3000 2325 3150 2025 2850 2025 3000 2325
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 2700 3075 2550 3375 2850 3375 2700 3075
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 3300 3075 3150 3375 3450 3375 3300 3075
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 5100 2400 5250 2100 4950 2100 5100 2400
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 6900 3075 6750 3375 7050 3375 6900 3075
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 4800 3075 4650 3375 4950 3375 4800 3075
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 5400 3075 5250 3375 5550 3375 5400 3075
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 7500 3075 7350 3375 7650 3375 7500 3075
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 9030 3015 8880 3315 9180 3315 9030 3015
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 9630 3015 9480 3315 9780 3315 9630 3015
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 11100 3075 10950 3375 11250 3375 11100 3075
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 11700 3075 11550 3375 11850 3375 11700 3075
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 13200 3075 13050 3375 13350 3375 13200 3075
	 0.000 -1.000 -1.000 0.000
4 0 0 50 0 0 12 0.0000 4 45 105 9900 4575 =\001
4 0 0 50 0 0 15 0.0000 4 195 255 2925 1575 [3]\001
4 0 0 50 0 0 15 0.0000 4 195 255 4950 1575 [6]\001
4 0 0 50 0 0 15 0.0000 4 195 255 7050 1575 [6]\001
4 0 0 50 0 0 15 0.0000 4 195 255 9150 1575 [6]\001
4 0 0 50 0 0 15 0.0000 4 195 255 13425 1575 [3]\001
4 0 0 50 0 0 15 0.0000 4 195 255 11325 1575 [6]\001


==> figures/b3edges <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 3000 2400 75 75 3000 2400 3000 2475
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 2700 3000 75 75 2700 3000 2700 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 3300 3000 75 75 3300 3000 3300 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 5100 2400 75 75 5100 2400 5100 2475
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 4800 3000 75 75 4800 3000 4800 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 5400 3000 75 75 5400 3000 5400 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 7200 2400 75 75 7200 2400 7200 2475
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 6900 3000 75 75 6900 3000 6900 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 7500 3000 75 75 7500 3000 7500 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 9300 2400 75 75 9300 2400 9300 2475
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 9600 3000 75 75 9600 3000 9600 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 9000 3000 75 75 9000 3000 9000 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 11400 2400 75 75 11400 2400 11400 2475
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 11100 3000 75 75 11100 3000 11100 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 11700 3000 75 75 11700 3000 11700 3075
2 1 1 3 0 7 50 0 -1 8.000 0 0 -1 0 0 5
	 2400 1800 2400 3600 3600 3600 3600 1800 2400 1800
2 1 1 3 0 7 50 0 -1 8.000 0 0 -1 0 0 5
	 4500 1800 4500 3600 5700 3600 5700 1800 4500 1800
2 1 1 3 0 7 50 0 -1 8.000 0 0 -1 0 0 5
	 6600 1800 6600 3600 7800 3600 7800 1800 6600 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 2775 3000 3225 3000
2 1 1 3 0 7 50 0 -1 8.000 0 0 -1 0 0 5
	 8700 1800 8700 3600 9900 3600 9900 1800 8700 1800
2 1 1 3 0 7 50 0 -1 8.000 0 0 -1 0 0 5
	 10800 1800 10800 3600 12000 3600 12000 1800 10800 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 5400 2925 5175 2475
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 5025 2475 4800 2925
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 9600 4500 9000 4500
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 10875 4500 10350 4500
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 10350 4650 10950 4650
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 8700 4200 8700 4800 11400 4800 11400 4200 8700 4200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 4875 3000 5325 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 7275 2475 7500 2925
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 6975 3000 7425 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 9075 3000 9525 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 11175 3000 11625 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 11475 2475 11700 2925
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 9225 2475 9000 2925
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 9600 2925 9375 2400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 11100 2925 11400 2475
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 3000 2325 3150 2025 2850 2025 3000 2325
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 2700 3075 2550 3375 2850 3375 2700 3075
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 3300 3075 3150 3375 3450 3375 3300 3075
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 5100 2400 5250 2100 4950 2100 5100 2400
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 6900 3075 6750 3375 7050 3375 6900 3075
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 4800 3075 4650 3375 4950 3375 4800 3075
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 5400 3075 5250 3375 5550 3375 5400 3075
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 7200 2325 7350 2025 7050 2025 7200 2325
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 9300 2325 9450 2025 9150 2025 9300 2325
	 0.000 -1.000 -1.000 0.000
4 0 0 50 0 0 12 0.0000 4 45 105 9900 4575 =\001
4 0 0 50 0 0 15 0.0000 4 195 255 2925 1575 [3]\001
4 0 0 50 0 0 15 0.0000 4 195 255 5025 1575 [2]\001
4 0 0 50 0 0 15 0.0000 4 195 255 7125 1575 [3]\001
4 0 0 50 0 0 15 0.0000 4 195 255 9225 1575 [6]\001
4 0 0 50 0 0 15 0.0000 4 195 255 11325 1575 [1]\001


==> figures/b3facets <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 3000 2400 75 75 3000 2400 3000 2475
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 2700 3000 75 75 2700 3000 2700 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 3300 3000 75 75 3300 3000 3300 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 5100 2400 75 75 5100 2400 5100 2475
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 4800 3000 75 75 4800 3000 4800 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 5400 3000 75 75 5400 3000 5400 3075
2 1 1 3 0 7 50 0 -1 8.000 0 0 -1 0 0 5
	 2400 1800 2400 3600 3600 3600 3600 1800 2400 1800
2 1 1 3 0 7 50 0 -1 8.000 0 0 -1 0 0 5
	 4500 1800 4500 3600 5700 3600 5700 1800 4500 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 2775 3000 3225 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 5175 2475 5400 2925
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 4783 2913 5083 2463
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 4875 3000 5325 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 2666 2901 2966 2451
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 3075 2475 3300 2925
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 6525 2700 6525 3300 9225 3300 9225 2700 6525 2700
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 7350 3000 6750 3000
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 8625 2925 8100 2925
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 8100 3075 8700 3075
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 3000 2325 3150 2025 2850 2025 3000 2325
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 2700 3075 2550 3375 2850 3375 2700 3075
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 3300 3075 3150 3375 3450 3375 3300 3075
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 4800 3075 4650 3375 4950 3375 4800 3075
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 4
	0 0 1.00 60.00 120.00
	 5400 3075 5250 3375 5550 3375 5400 3075
	 0.000 -1.000 -1.000 0.000
4 0 0 50 0 0 12 0.0000 4 45 105 7650 3075 =\001
4 0 0 50 0 0 15 0.0000 4 195 255 2925 1575 [6]\001
4 0 0 50 0 0 15 0.0000 4 195 255 5025 1575 [3]\001


==> figures/colorcubehilbertbasis <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 1200 6000 150 150 1200 6000 1350 6000
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 4800 6000 150 150 4800 6000 4800 6150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 3000 4200 150 150 3000 4200 3000 4350
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 4800 4200 150 150 4800 4200 4950 4200
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 1200 2400 150 150 1200 2400 1200 2550
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 3000 2400 150 150 3000 2400 3150 2400
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 1769 5369 150 150 1769 5369 1769 5519
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 3600 5400 150 150 3600 5400 3750 5400
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 4200 4800 150 150 4200 4800 4200 4950
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 2444 1231 150 150 2444 1231 2594 1231
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 3600 1800 150 150 3600 1800 3600 1950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 2400 3000 150 150 2400 3000 2400 3150
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 1800 3600 150 150 1800 3600 1950 3600
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 6000 1200 150 150 6000 1200 6000 1350
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 5400 1800 150 150 5400 1800 5550 1800
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 4200 3000 150 150 4200 3000 4350 3000
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 5400 3600 150 150 5400 3600 5400 3750
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 6000 4800 150 150 6000 4800 6150 4800
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 11400 4200 150 150 11400 4200 11550 4200
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 11400 2400 150 150 11400 2400 11400 2550
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 9600 2400 150 150 9600 2400 9750 2400
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 9600 4200 150 150 9600 4200 9600 4350
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 10800 3000 150 150 10800 3000 10950 3000
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 12000 1800 150 150 12000 1800 12150 1800
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 10200 1800 150 150 10200 1800 10200 1950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 8400 5400 150 150 8400 5400 8400 5550
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 9000 4800 150 150 9000 4800 9150 4800
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 10800 4800 150 150 10800 4800 10800 4950
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 10200 5400 150 150 10200 5400 10350 5400
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 12000 3600 150 150 12000 3600 12000 3750
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 8400 3600 150 150 8400 3600 8550 3600
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 9031 3031 150 150 9031 3031 9031 3181
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 2400 7800 150 150 2400 7800 2550 7800
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 6000 7800 150 150 6000 7800 6000 7950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 2400 11400 150 150 2400 11400 2400 11550
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 6000 11400 150 150 6000 11400 6150 11400
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 4756 12631 150 150 4756 12631 4756 12781
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 1169 12631 150 150 1169 12631 1319 12631
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 1200 9000 150 150 1200 9000 1200 9150
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 4800 9000 150 150 4800 9000 4950 9000
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 12600 13200 150 150 12600 13200 12600 13350
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 12600 14400 150 150 12600 14400 12750 14400
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 6000 3000 150 150 6000 3000 6000 3150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 4200 1200 150 150 4200 1200 4200 1350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 1800 1800 150 150 1800 1800 1800 1950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 1200 4200 150 150 1200 4200 1200 4350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 2400 4800 150 150 2400 4800 2400 4950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 3000 6000 150 150 3000 6000 3000 6150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 4800 2400 150 150 4800 2400 4800 2550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 5400 5400 150 150 5400 5400 5400 5550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 3600 3525 150 150 3600 3525 3600 3675
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 8400 1800 150 150 8400 1800 8400 1950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 9000 1275 150 150 9000 1275 9000 1425
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 7875 2400 150 150 7875 2400 7875 2550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 10800 1200 150 150 10800 1200 10800 1350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 12525 1275 150 150 12525 1275 12525 1425
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 12600 3000 150 150 12600 3000 12600 3150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 12600 4800 150 150 12600 4800 12600 4950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 12000 5400 150 150 12000 5400 12000 5550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 11400 6000 150 150 11400 6000 11400 6150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 9600 6000 150 150 9600 6000 9600 6150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 7875 5925 150 150 7875 5925 7875 6075
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 7800 4200 150 150 7800 4200 7800 4350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 10200 3600 150 150 10200 3600 10200 3750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 1800 8400 150 150 1800 8400 1800 8550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 4125 7800 150 150 4125 7800 4125 7950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 3600 8400 150 150 3600 8400 3600 8550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 12600 13800 150 150 12600 13800 12600 13950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 2400 9600 150 150 2400 9600 2400 9750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 3000 9000 150 150 3000 9000 3000 9150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 3600 10200 150 150 3600 10200 3600 10350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 4200 9525 150 150 4200 9525 4200 9675
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 6000 9600 150 150 6000 9600 6000 9750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 5400 10200 150 150 5400 10200 5400 10350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 4800 10800 150 150 4800 10800 4800 10950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 5325 12000 150 150 5325 12000 5325 12150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 3675 12000 150 150 3675 12000 3675 12150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 3000 12600 150 150 3000 12600 3000 12750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 4200 11400 150 150 4200 11400 4200 11550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 1800 12000 150 150 1800 12000 1800 12150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 1200 10800 150 150 1200 10800 1200 10950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 1800 10200 150 150 1800 10200 1800 10350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 5400 8400 150 150 5400 8400 5400 8550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 3000 10800 150 150 3000 10800 3000 10950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 7800 10800 150 150 7800 10800 7800 10950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 8400 10200 150 150 8400 10200 8400 10350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 9000 9600 150 150 9000 9600 9000 9750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 7875 9000 150 150 7875 9000 7875 9150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 8400 8400 150 150 8400 8400 8400 8550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 9000 7800 150 150 9000 7800 9000 7950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 10800 7800 150 150 10800 7800 10800 7950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 10200 8400 150 150 10200 8400 10200 8550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 9600 9000 150 150 9600 9000 9600 9150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 11325 9000 150 150 11325 9000 11325 9150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 12000 8475 150 150 12000 8475 12000 8625
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 12525 7875 150 150 12525 7875 12525 8025
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 12600 9600 150 150 12600 9600 12600 9750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 12000 10200 150 150 12000 10200 12000 10350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 11400 10800 150 150 11400 10800 11400 10950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 12000 12000 150 150 12000 12000 12000 12150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 12600 11400 150 150 12600 11400 12600 11550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 11400 12600 150 150 11400 12600 11400 12750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 10800 11400 150 150 10800 11400 10800 11550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 10200 12000 150 150 10200 12000 10200 12150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 9600 12600 150 150 9600 12600 9600 12750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 7875 12525 150 150 7875 12525 7875 12675
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 8400 11925 150 150 8400 11925 8400 12075
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 9075 11325 150 150 9075 11325 9075 11475
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 9600 10800 150 150 9600 10800 9600 10950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 10200 10200 150 150 10200 10200 10200 10350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 10800 9600 150 150 10800 9600 10800 9750
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1350 6000 2850 6000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3225 6000 4650 6000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 4350 1200 5850
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 4050 1200 2550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1350 2400 2850 2400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3150 2400 4650 2400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 4050 4800 2550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 5850 4800 4350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4350 1200 5850 1200
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2550 1200 4050 1200
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5550 1650 5925 1275
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4875 2250 5250 1875
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 1425 2400 2775
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 4650 2400 3150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1275 5850 1650 5475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1875 5250 2325 4800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2550 4800 4050 4800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4350 4800 5850 4800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5550 5325 6000 4875
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4950 5925 5325 5550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 2850 6000 1350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 4650 6000 3150
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5400 3450 5400 2025
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5400 5175 5400 3750
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5550 3525 5925 3150
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1350 4050 1725 3675
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1950 3450 2325 3075
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1800 3375 1800 1950
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1800 5175 1800 3750
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1950 5400 3450 5400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3750 5400 5250 5400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3150 5850 3525 5475
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3712 5287 4087 4912
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4950 4050 5325 3675
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4200 2775 4200 1350
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4200 4575 4200 3150
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 2550 3000 4050 3000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4350 3000 5850 3000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1950 1800 3450 1800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3750 1800 5250 1800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1950 3600 3450 3600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1950 3600 3450 3600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3750 3600 5250 3600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3600 3375 3600 1950
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3600 5175 3600 3750
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1350 4200 2850 4200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3150 4200 4650 4200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3000 3975 3000 2550
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3000 5775 3000 4350
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3075 2250 3450 1875
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3712 1687 4087 1312
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 4050 7800 2550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 5850 7800 4350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7950 2400 9450 2400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9750 2400 11250 2400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7950 6000 9450 6000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9750 6000 11250 6000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11400 4050 11400 2550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11400 5850 11400 4350
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9600 2550 9600 4050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9600 4350 9600 5850
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1312 2287 1687 1912
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1912 1687 2287 1312
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7912 2212 8287 1837
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11512 2287 11887 1912
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9150 1200 10650 1200
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10950 1200 12450 1200
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12112 1687 12487 1312
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8512 1687 8887 1312
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8550 1800 10050 1800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10350 1800 11850 1800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10312 1687 10687 1312
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9712 2287 10087 1912
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12600 2850 12600 1350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12600 4650 12600 3150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12112 5362 12562 4912
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11512 5962 11962 5512
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8475 5325 8925 4875
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7875 5925 8325 5475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9150 4800 10650 4800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10950 4800 12450 4800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10312 5287 10687 4912
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9712 5887 10087 5512
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8550 5400 10050 5400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10350 5400 11850 5400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8400 1950 8400 3450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8400 3750 8400 5250
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 12000 1950 12000 3450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 12000 3750 12000 5250
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 11512 4087 11887 3712
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 12112 3487 12487 3112
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 7912 4087 8287 3712
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8587 3487 8962 3112
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 1425 9000 2775
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 3225 9000 4575
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 7950 4200 9450 4200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9750 4200 11250 4200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10800 1350 10800 2850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10800 3150 10800 4650
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9150 3000 10650 3000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10950 3000 12450 3000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8550 3600 10050 3600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10350 3600 11850 3600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10200 1950 10200 3450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10200 3750 10200 5250
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 11250 6000 9750
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 9450 6000 7950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 9450 2400 7950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 11250 2400 9750
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2550 7800 4050 7800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4350 7800 5850 7800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4350 11400 5850 11400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2550 11400 4050 11400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5475 11925 5925 11475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1875 11925 2325 11475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4837 12562 5287 12112
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1275 12525 1725 12075
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3150 12600 4650 12600
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1350 12600 2850 12600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3150 12525 3525 12150
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3750 11925 4125 11550
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4200 9750 4200 11250
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4200 7875 4200 9375
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1950 12000 3450 12000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3825 12000 5325 12000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 12450 4800 10950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 12450 1200 10950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 10650 4800 9150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 10650 1200 9150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1350 9000 2850 9000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3150 9000 4650 9000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1312 8887 1762 8437
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1912 8287 2362 7837
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5512 8287 5962 7837
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4912 8887 5362 8437
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3675 8250 4050 7875
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3075 8850 3450 8475
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1950 8400 3450 8400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3750 8400 5250 8400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5400 8550 5400 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5400 10350 5400 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4912 10687 5287 10312
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5512 10087 5887 9712
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1800 8550 1800 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1800 10350 1800 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1350 10800 2850 10800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3150 10800 4650 10800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3000 9150 3000 10650
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3000 10950 3000 12450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3600 8550 3600 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3600 10350 3600 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 2550 9600 4050 9600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4350 9600 5850 9600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1312 10687 1687 10312
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1912 10087 2287 9712
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 10650 7800 9150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11400 12450 11400 10950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11400 10650 11400 9150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 12450 7800 10950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7950 9000 9450 9000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9750 9000 11250 9000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9750 12600 11250 12600
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7950 12600 9450 12600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9600 9150 9600 10650
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9600 10950 9600 12450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 7950 10800 9450 10800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9750 10800 11250 10800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11512 12562 11962 12112
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12112 11962 12562 11512
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9150 11400 10650 11400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10950 11400 12450 11400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7837 12487 8287 12037
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8512 11887 8962 11437
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12600 11250 12600 9750
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12600 9450 12600 7950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11475 8925 11925 8475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12075 8325 12525 7875
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10950 7800 12450 7800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9150 7800 10650 7800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8437 8287 8887 7837
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7912 8887 8362 8437
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 9450 9000 7950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 11250 9000 9750
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10800 7950 10800 9450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10800 9750 10800 11250
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9150 9600 10650 9600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10950 9600 12450 9600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8400 8550 8400 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8400 10350 8400 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8550 12000 10050 12000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10350 12000 11850 12000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 12000 8550 12000 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 12000 10350 12000 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8550 8400 10050 8400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10350 8400 11850 8400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10275 8250 10650 7875
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9675 8850 10050 8475
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8550 10050 8925 9675
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 7950 10650 8325 10275
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 11512 10687 11887 10312
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 12112 10087 12487 9712
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10200 10350 10200 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10200 8550 10200 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8625 10200 10125 10200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10350 10200 11850 10200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9675 12450 10050 12075
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10275 11850 10650 11475
4 0 0 50 0 0 20 0.0000 4 240 315 4050 900 [8]\001
4 0 0 50 0 0 20 0.0000 4 240 315 10650 900 [8]\001
4 0 0 50 0 0 20 0.0000 4 240 315 4050 7500 [2]\001
4 0 0 50 0 0 20 0.0000 4 240 315 10650 7500 [1]\001
4 0 0 50 0 0 20 0.0000 4 195 135 13125 13275 0\001
4 0 0 50 0 0 20 0.0000 4 195 135 13125 13875 1\001
4 0 0 50 0 0 20 0.0000 4 195 135 13125 14475 2\001
4 0 0 50 0 0 20 0.0000 4 195 1305 12300 12825 Label  code\001


==> figures/colorsemicubehilbertbasis <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 12600 13200 150 150 12600 13200 12600 13350
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 12600 14400 150 150 12600 14400 12750 14400
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 1200 6000 150 150 1200 6000 1200 6150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 3000 6000 150 150 3000 6000 3000 6150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 3000 4200 150 150 3000 4200 3000 4350
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 1275 2400 150 150 1275 2400 1275 2550
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 4800 2400 150 150 4800 2400 4800 2550
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 3600 5325 150 150 3600 5325 3600 5475
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 5400 5400 150 150 5400 5400 5400 5550
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 1800 3525 150 150 1800 3525 1800 3675
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 1800 1800 150 150 1800 1800 1800 1950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 2400 3000 150 150 2400 3000 2400 3150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 2400 4800 150 150 2400 4800 2400 4950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 5400 3600 150 150 5400 3600 5400 3750
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 3600 1875 150 150 3600 1875 3600 2025
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 4200 1200 150 150 4200 1200 4200 1350
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 5925 1200 150 150 5925 1200 5925 1350
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 6000 4800 150 150 6000 4800 6000 4950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 4800 4200 150 150 4800 4200 4800 4350
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 4200 3000 150 150 4200 3000 4200 3150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 7800 6000 150 150 7800 6000 7800 6150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 9600 6000 150 150 9600 6000 9600 6150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 7844 4169 150 150 7844 4169 7844 4319
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 11369 4169 150 150 11369 4169 11369 4319
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 11369 2444 150 150 11369 2444 11369 2594
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 9569 2444 150 150 9569 2444 9569 2594
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 8400 5400 150 150 8400 5400 8400 5550
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 10800 4800 150 150 10800 4800 10800 4950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 12600 4800 150 150 12600 4800 12600 4950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 12000 5400 150 150 12000 5400 12000 5550
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 10156 3631 150 150 10156 3631 10156 3781
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 12031 3631 150 150 12031 3631 12031 3781
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 8431 1831 150 150 8431 1831 8431 1981
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 10200 1875 150 150 10200 1875 10200 2025
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 9000 3000 150 150 9000 3000 9000 3150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 10800 3000 150 150 10800 3000 10800 3150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 9000 1200 150 150 9000 1200 9000 1350
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 12525 1275 150 150 12525 1275 12525 1425
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -2431 2969 150 150 -2431 2969 -2431 3119
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -631 1244 150 150 -631 1244 -631 1394
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -4169 4769 150 150 -4169 4769 -4169 4919
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -5400 6000 150 150 -5400 6000 -5250 6000
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -3600 6000 150 150 -3600 6000 -3600 6150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -1800 6000 150 150 -1800 6000 -1800 6150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -5431 2431 150 150 -5431 2431 -5431 2581
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -5400 4200 150 150 -5400 4200 -5400 4350
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -4800 5400 150 150 -4800 5400 -4800 5550
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -1200 3600 150 150 -1200 3600 -1200 3750
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -3000 1800 150 150 -3000 1800 -3000 1950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -10800 4800 150 150 -10800 4800 -10800 4950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -9000 1200 150 150 -9000 1200 -9000 1350
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -7200 3000 150 150 -7200 3000 -7200 3150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -11400 5400 150 150 -11400 5400 -11400 5550
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -9600 3600 150 150 -9600 3600 -9600 3750
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -7800 1800 150 150 -7800 1800 -7800 1950
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -12000 6000 150 150 -12000 6000 -11850 6000
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -10200 6000 150 150 -10200 6000 -10200 6150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -8400 6000 150 150 -8400 6000 -8400 6150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -12000 4200 150 150 -12000 4200 -12000 4350
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -12000 2400 150 150 -12000 2400 -12000 2550
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -2400 11400 150 150 -2400 11400 -2400 11550
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -4231 9631 150 150 -4231 9631 -4231 9781
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -600 7800 150 150 -600 7800 -600 7950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -5400 12600 150 150 -5400 12600 -5400 12750
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -5400 10800 150 150 -5400 10800 -5250 10800
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -3631 10769 150 150 -3631 10769 -3631 10919
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -1800 10800 150 150 -1800 10800 -1800 10950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -5400 9000 150 150 -5400 9000 -5400 9150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -1200 12000 150 150 -1200 12000 -1200 12150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -4800 10200 150 150 -4800 10200 -4800 10350
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -3000 8400 150 150 -3000 8400 -3000 8550
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 1800 10200 150 150 1800 10200 1950 10200
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 3600 10200 150 150 3600 10200 3600 10350
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 5400 10200 150 150 5400 10200 5400 10350
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 1200 10800 150 150 1200 10800 1200 10950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 3000 12600 150 150 3000 12600 3000 12750
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 4800 9000 150 150 4800 9000 4800 9150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 1800 8400 150 150 1800 8400 1800 8550
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 2369 9631 150 150 2369 9631 2369 9781
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 5969 11356 150 150 5969 11356 5969 11506
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 4211 7817 150 150 4211 7817 4211 7967
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 10200 10200 150 150 10200 10200 10350 10200
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 8400 10200 150 150 8400 10200 8400 10350
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 12000 10200 150 150 12000 10200 12000 10350
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 10200 8400 150 150 10200 8400 10200 8550
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 10200 11925 150 150 10200 11925 10200 12075
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 9600 10800 150 150 9600 10800 9600 10950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 10800 9600 150 150 10800 9600 10800 9750
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 7800 12600 150 150 7800 12600 7800 12750
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 11400 9000 150 150 11400 9000 11400 9150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 9000 7800 150 150 9000 7800 9000 7950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 12600 11400 150 150 12600 11400 12600 11550
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 1844 11969 150 150 1844 11969 1844 12119
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -12000 12600 150 150 -12000 12600 -12000 12750
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -12000 10800 150 150 -12000 10800 -11850 10800
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -10200 10800 150 150 -10200 10800 -10200 10950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -8400 10800 150 150 -8400 10800 -8400 10950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -12000 9000 150 150 -12000 9000 -12000 9150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -9600 12000 150 150 -9600 12000 -9600 12150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -11400 10200 150 150 -11400 10200 -11400 10350
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -9000 7800 150 150 -9000 7800 -9000 7950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -7231 11369 150 150 -7231 11369 -7231 11519
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -10769 9631 150 150 -10769 9631 -10769 9781
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -7831 8444 150 150 -7831 8444 -7831 8594
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -675 4800 150 150 -675 4800 -675 4950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -1200 5400 150 150 -1200 5400 -1200 5550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -3000 5400 150 150 -3000 5400 -3000 5550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -2400 4800 150 150 -2400 4800 -2400 4950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -4800 3600 150 150 -4800 3600 -4800 3750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -4200 3000 150 150 -4200 3000 -4200 3150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -4875 1800 150 150 -4875 1800 -4875 1950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -4200 1200 150 150 -4200 1200 -4200 1350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -2400 1200 150 150 -2400 1200 -2400 1350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -3600 2400 150 150 -3600 2400 -3600 2550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -1800 2400 150 150 -1800 2400 -1800 2550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -1200 1800 150 150 -1200 1800 -1200 1950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -3600 4125 150 150 -3600 4125 -3600 4275
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -3000 3600 150 150 -3000 3600 -3000 3750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -1800 4200 150 150 -1800 4200 -1800 4350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -600 3000 150 150 -600 3000 -600 3150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -10800 1200 150 150 -10800 1200 -10800 1350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -11400 1800 150 150 -11400 1800 -11400 1950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -10200 2400 150 150 -10200 2400 -10200 2550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -9600 1800 150 150 -9600 1800 -9600 1950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -8400 2400 150 150 -8400 2400 -8400 2550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -7275 1275 150 150 -7275 1275 -7275 1425
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -7800 3525 150 150 -7800 3525 -7800 3675
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -8400 4200 150 150 -8400 4200 -8400 4350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -7800 5400 150 150 -7800 5400 -7800 5550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -7200 4800 150 150 -7200 4800 -7200 4950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -9600 5400 150 150 -9600 5400 -9600 5550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -10800 3000 150 150 -10800 3000 -10800 3150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -11400 3600 150 150 -11400 3600 -11400 3750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -10200 4200 150 150 -10200 4200 -10200 4350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -9000 4800 150 150 -9000 4800 -9000 4950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 1800 5400 150 150 1800 5400 1800 5550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 1200 4200 150 150 1200 4200 1200 4350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 2400 1275 150 150 2400 1275 2400 1425
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 3000 2400 150 150 3000 2400 3000 2550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 5400 1800 150 150 5400 1800 5400 1950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 6000 3000 150 150 6000 3000 6000 3150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 4200 4725 150 150 4200 4725 4200 4875
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 4800 6000 150 150 4800 6000 4800 6150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 3600 3600 150 150 3600 3600 3600 3750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 9000 4800 150 150 9000 4800 9000 4950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 8400 3600 150 150 8400 3600 8400 3750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 7800 2400 150 150 7800 2400 7800 2550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 10725 1200 150 150 10725 1200 10725 1350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 12000 1800 150 150 12000 1800 12000 1950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 12600 3000 150 150 12600 3000 12600 3150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 9600 4200 150 150 9600 4200 9600 4350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 10200 5400 150 150 10200 5400 10200 5550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 11325 6000 150 150 11325 6000 11325 6150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 12600 7875 150 150 12600 7875 12600 8025
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 12000 8400 150 150 12000 8400 12000 8550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 12600 9600 150 150 12600 9600 12600 9750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 11400 10800 150 150 11400 10800 11400 10950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 11925 12000 150 150 11925 12000 11925 12150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 11325 12600 150 150 11325 12600 11325 12750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 9600 12600 150 150 9600 12600 9600 12750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 8400 12000 150 150 8400 12000 8400 12150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 9075 11400 150 150 9075 11400 9075 11550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 7800 10800 150 150 7800 10800 7800 10950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 9000 9600 150 150 9000 9600 9000 9750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 7800 9000 150 150 7800 9000 7800 9150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 8475 8400 150 150 8475 8400 8475 8550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 10800 7800 150 150 10800 7800 10800 7950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 9600 9000 150 150 9600 9000 9600 9150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 10800 11400 150 150 10800 11400 10800 11550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 12600 13800 150 150 12600 13800 12600 13950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 5400 12000 150 150 5400 12000 5400 12150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 4800 12600 150 150 4800 12600 4800 12750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 4200 11400 150 150 4200 11400 4200 11550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 2400 11400 150 150 2400 11400 2400 11550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 3000 10800 150 150 3000 10800 3000 10950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 4800 10800 150 150 4800 10800 4800 10950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 6000 9600 150 150 6000 9600 6000 9750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 4200 9600 150 150 4200 9600 4200 9750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 2400 7800 150 150 2400 7800 2400 7950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 3000 9000 150 150 3000 9000 3000 9150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 3525 8400 150 150 3525 8400 3525 8550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 5400 8400 150 150 5400 8400 5400 8550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 5925 7875 150 150 5925 7875 5925 8025
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 1275 9000 150 150 1275 9000 1275 9150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -3600 12600 150 150 -3600 12600 -3600 12750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -3000 12000 150 150 -3000 12000 -3000 12150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -1800 12600 150 150 -1800 12600 -1800 12750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -600 11400 150 150 -600 11400 -600 11550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -4200 11400 150 150 -4200 11400 -4200 11550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -4800 12000 150 150 -4800 12000 -4800 12150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -4800 8400 150 150 -4800 8400 -4800 8550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -4200 7800 150 150 -4200 7800 -4200 7950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -2400 7800 150 150 -2400 7800 -2400 7950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -3600 9000 150 150 -3600 9000 -3600 9150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -1875 9000 150 150 -1875 9000 -1875 9150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -1200 8400 150 150 -1200 8400 -1200 8550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -600 9600 150 150 -600 9600 -600 9750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -1200 10200 150 150 -1200 10200 -1200 10350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -2400 9600 150 150 -2400 9600 -2400 9750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -3000 10200 150 150 -3000 10200 -3000 10350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -8400 12600 150 150 -8400 12600 -8400 12750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -7800 10200 150 150 -7800 10200 -7800 10350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -7275 7875 150 150 -7275 7875 -7275 8025
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -8400 9000 150 150 -8400 9000 -8400 9150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -9000 9600 150 150 -9000 9600 -9000 9750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -9600 10200 150 150 -9600 10200 -9600 10350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -11475 12000 150 150 -11475 12000 -11475 12150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -10800 11400 150 150 -10800 11400 -10800 11550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -9000 11400 150 150 -9000 11400 -9000 11550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -10200 12600 150 150 -10200 12600 -10200 12750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -10800 7800 150 150 -10800 7800 -10800 7950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -11400 8325 150 150 -11400 8325 -11400 8475
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -10200 9000 150 150 -10200 9000 -10200 9150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -9600 8400 150 150 -9600 8400 -9600 8550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -7125 9600 150 150 -7125 9600 -7125 9750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -7800 12000 150 150 -7800 12000 -7800 12150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 1200 12600 150 150 1200 12600 1200 12750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 3600 12000 150 150 3600 12000 3600 12150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1350 6000 2850 6000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3225 6000 4650 6000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 4350 1200 5850
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 4050 1200 2550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1350 2400 2850 2400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3150 2400 4650 2400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 4050 4800 2550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 5850 4800 4350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4350 1200 5850 1200
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2550 1200 4050 1200
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5550 1650 5925 1275
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4875 2250 5250 1875
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 4650 2400 3150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1275 5850 1650 5475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1875 5250 2325 4800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2550 4800 4050 4800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4350 4800 5850 4800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5550 5325 6000 4875
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4950 5925 5325 5550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 2850 6000 1350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 4650 6000 3150
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5400 3450 5400 2025
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5400 5175 5400 3750
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5550 3525 5925 3150
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1350 4050 1725 3675
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1950 3450 2325 3075
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1800 3375 1800 1950
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1800 5175 1800 3750
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1950 5400 3450 5400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3750 5400 5250 5400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3150 5850 3525 5475
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3712 5287 4087 4912
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4950 4050 5325 3675
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4200 2775 4200 1350
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4200 4575 4200 3150
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 2550 3000 4050 3000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4350 3000 5850 3000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3750 1800 5250 1800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1950 3600 3450 3600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1950 3600 3450 3600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3750 3600 5250 3600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3600 3375 3600 1950
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3600 5175 3600 3750
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1350 4200 2850 4200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3150 4200 4650 4200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3000 3975 3000 2550
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3000 5775 3000 4350
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3075 2250 3450 1875
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3712 1687 4087 1312
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 4050 7800 2550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 5850 7800 4350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7950 2400 9450 2400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9750 2400 11250 2400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7950 6000 9450 6000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9750 6000 11250 6000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11400 4050 11400 2550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11400 5850 11400 4350
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9600 2550 9600 4050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9600 4350 9600 5850
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1312 2287 1687 1912
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1912 1687 2287 1312
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7912 2212 8287 1837
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11512 2287 11887 1912
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9150 1200 10650 1200
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10950 1200 12450 1200
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12112 1687 12487 1312
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8512 1687 8887 1312
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8550 1800 10050 1800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10350 1800 11850 1800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10312 1687 10687 1312
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9712 2287 10087 1912
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12600 2850 12600 1350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12600 4650 12600 3150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12112 5362 12562 4912
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11512 5962 11962 5512
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8475 5325 8925 4875
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7875 5925 8325 5475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9150 4800 10650 4800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10950 4800 12450 4800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10312 5287 10687 4912
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9712 5887 10087 5512
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8550 5400 10050 5400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10350 5400 11850 5400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8400 1950 8400 3450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8400 3750 8400 5250
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 12000 1950 12000 3450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 12000 3750 12000 5250
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 11512 4087 11887 3712
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 12112 3487 12487 3112
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 7912 4087 8287 3712
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8587 3487 8962 3112
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 1425 9000 2775
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 3225 9000 4575
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 7950 4200 9450 4200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9750 4200 11250 4200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10800 1350 10800 2850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10800 3150 10800 4650
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10950 3000 12450 3000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8550 3600 10050 3600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10350 3600 11850 3600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10200 1950 10200 3450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10200 3750 10200 5250
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 11250 6000 9750
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 9450 6000 7950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 9450 2400 7950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 11250 2400 9750
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2550 7800 4050 7800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4350 7800 5850 7800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4350 11400 5850 11400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2550 11400 4050 11400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5475 11925 5925 11475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1875 11925 2325 11475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4837 12562 5287 12112
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1275 12525 1725 12075
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3150 12600 4650 12600
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1350 12600 2850 12600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3150 12525 3525 12150
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3750 11925 4125 11550
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4200 9750 4200 11250
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4200 7875 4200 9375
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1950 12000 3450 12000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3825 12000 5325 12000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 12450 4800 10950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 12450 1200 10950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 10650 4800 9150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 10650 1200 9150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1350 9000 2850 9000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3150 9000 4650 9000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1312 8887 1762 8437
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1912 8287 2362 7837
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5512 8287 5962 7837
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4912 8887 5362 8437
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3675 8250 4050 7875
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3075 8850 3450 8475
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1950 8400 3450 8400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3750 8400 5250 8400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5400 8550 5400 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5400 10350 5400 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4912 10687 5287 10312
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5512 10087 5887 9712
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1800 8550 1800 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1800 10350 1800 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1350 10800 2850 10800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3150 10800 4650 10800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3000 9150 3000 10650
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3000 10950 3000 12450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3600 8550 3600 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3600 10350 3600 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 2550 9600 4050 9600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4350 9600 5850 9600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1312 10687 1687 10312
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1912 10087 2287 9712
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 10650 7800 9150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11400 12450 11400 10950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11400 10650 11400 9150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 12450 7800 10950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7950 9000 9450 9000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9750 9000 11250 9000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9750 12600 11250 12600
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7950 12600 9450 12600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9600 9150 9600 10650
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9600 10950 9600 12450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 7950 10800 9450 10800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9750 10800 11250 10800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9150 11400 10650 11400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10950 11400 12450 11400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7837 12487 8287 12037
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8512 11887 8962 11437
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12600 11250 12600 9750
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12600 9450 12600 7950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11475 8925 11925 8475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10950 7800 12450 7800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9150 7800 10650 7800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 9450 9000 7950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 11250 9000 9750
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10800 7950 10800 9450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10800 9750 10800 11250
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9150 9600 10650 9600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10950 9600 12450 9600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8400 8550 8400 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8400 10350 8400 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8550 12000 10050 12000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10350 12000 11850 12000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 12000 8550 12000 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 12000 10350 12000 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8550 8400 10050 8400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10350 8400 11850 8400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10275 8250 10650 7875
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9675 8850 10050 8475
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8550 10050 8925 9675
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 7950 10650 8325 10275
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 11512 10687 11887 10312
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 12112 10087 12487 9712
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10200 10350 10200 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10200 8550 10200 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8625 10200 10125 10200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10350 10200 11850 10200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9675 12450 10050 12075
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 10275 11850 10650 11475
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1950 1800 3450 1800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 2850 2400 1350
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9150 3000 10650 3000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -600 2850 -600 1350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -600 4650 -600 3150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5250 6000 -3750 6000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -3450 6000 -1950 6000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5400 5850 -5400 4350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5400 4050 -5400 2550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1800 4050 -1800 2550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1800 5850 -1800 4350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5250 2400 -3750 2400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4050 4800 -2550 4800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -2250 4800 -750 4800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5325 5850 -4950 5475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4050 1200 -2550 1200
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -2250 1200 -750 1200
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4725 1650 -4350 1275
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5325 2250 -4950 1875
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4200 2850 -4200 1350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4200 4650 -4200 3150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4687 5212 -4312 4837
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1687 5887 -1312 5512
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1087 5287 -712 4912
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1724 2249 -1349 1874
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1049 1649 -674 1274
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -5250 4200 -3750 4200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3450 4200 -1950 4200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3000 5175 -3000 3750
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -1200 1950 -1200 3450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -1200 3750 -1200 5250
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4800 1950 -4800 3450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4800 3750 -4800 5250
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4650 5400 -3150 5400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2850 5400 -1350 5400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4650 1800 -3150 1800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2850 1800 -1350 1800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -5288 4087 -4913 3712
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4687 3487 -4312 3112
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -1687 4087 -1312 3712
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -1012 3487 -637 3112
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2887 5287 -2512 4912
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3487 5887 -3112 5512
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2887 1687 -2512 1312
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4050 3000 -2550 3000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2250 3000 -750 3000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2400 4575 -2400 3150
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2400 2775 -2400 1350
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4650 3600 -3150 3600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2850 3600 -1350 3600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3600 3975 -3600 2550
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3600 5775 -3600 4350
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3000 3375 -3000 1950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -3450 2400 -1950 2400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3524 2249 -3149 1874
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10650 1200 -9150 1200
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8850 1200 -7350 1200
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8850 4800 -7350 4800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10650 4800 -9150 4800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -7200 4650 -7200 3150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -7200 2850 -7200 1350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10800 2850 -10800 1350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10800 4650 -10800 3150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11850 6000 -10350 6000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10050 6000 -8550 6000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11850 2400 -10350 2400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10050 2400 -8550 2400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8400 4050 -8400 2550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8400 5850 -8400 4350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -12000 4050 -12000 2550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -12000 5850 -12000 4350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8287 5887 -7912 5512
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -7687 5287 -7312 4912
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11287 5287 -10912 4912
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11887 5887 -11512 5512
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11887 2287 -11512 1912
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11287 1687 -10912 1312
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8324 2249 -7949 1874
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -7724 1649 -7349 1274
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10124 2249 -9749 1874
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9524 1649 -9149 1274
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11924 4049 -11549 3674
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11324 3449 -10949 3074
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -7724 3449 -7349 3074
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10049 5849 -9674 5474
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9449 5249 -9074 4874
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -8286 4086 -7911 3711
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11250 3600 -9750 3600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9450 3600 -7950 3600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11250 1800 -9750 1800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9450 1800 -7950 1800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11250 5400 -9750 5400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9450 5400 -7950 5400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9600 1950 -9600 3450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9600 3750 -9600 5250
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11400 1950 -11400 3450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -7800 1950 -7800 3450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -7800 3750 -7800 5250
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11400 3750 -11400 5250
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10200 2550 -10200 4050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10200 4350 -10200 5850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11850 4200 -10350 4200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10050 4200 -8550 4200
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4050 7800 -2550 7800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -2250 7800 -750 7800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -600 9450 -600 7950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -600 11250 -600 9750
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4200 9450 -4200 7950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4200 11250 -4200 9750
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4050 11400 -2550 11400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -2250 11400 -750 11400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5250 9000 -3750 9000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -3450 12600 -1950 12600
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5250 12600 -3750 12600
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -3525 9000 -2025 9000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5400 10650 -5400 9150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5400 12450 -5400 10950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1800 10650 -1800 9150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1800 12450 -1800 10950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5325 8850 -4875 8400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4725 8250 -4275 7800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5325 12525 -4875 12075
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4725 11925 -4275 11475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1650 12525 -1200 12075
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1050 11925 -600 11475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1725 8925 -1275 8475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1125 8325 -675 7875
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4650 8400 -3150 8400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2925 8400 -1425 8400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2850 10200 -1350 10200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2850 12000 -1350 12000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4650 12000 -3150 12000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4650 10200 -3150 10200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3000 8550 -3000 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3000 10350 -3000 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2400 7950 -2400 9450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2400 9675 -2400 11175
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4800 8550 -4800 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4800 10350 -4800 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -1200 8550 -1200 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -1200 10350 -1200 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3488 12487 -3113 12112
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2887 11887 -2512 11512
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -1687 10687 -1312 10312
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -1087 10087 -712 9712
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -5287 10687 -4912 10312
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4687 10087 -4312 9712
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3487 8887 -3112 8512
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2887 8287 -2512 7912
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4050 9600 -2550 9600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2250 9600 -750 9600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3600 10950 -3600 12450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3600 9150 -3600 10650
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -5250 10800 -3750 10800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3450 10800 -1950 10800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12075 8325 12525 7875
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12075 11925 12525 11475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11437 12562 11887 12112
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8475 8325 8925 7875
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7912 8887 8362 8437
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10650 7800 -9150 7800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8850 7800 -7350 7800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10050 9000 -8550 9000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11850 9000 -10350 9000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11962 8887 -11512 8437
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11362 8287 -10912 7837
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -7687 8362 -7237 7912
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11250 8400 -9750 8400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9450 8400 -7950 8400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9524 8249 -9149 7874
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10124 8849 -9749 8474
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8400 10650 -8400 9150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -7200 9450 -7200 7950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -7200 11250 -7200 9750
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8400 12450 -8400 10950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -12000 10650 -12000 9150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -12000 12450 -12000 10950
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11850 10800 -10350 10800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10050 10800 -8550 10800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10200 9150 -10200 10650
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10200 10950 -10200 12450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11250 10200 -9750 10200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9450 10200 -7950 10200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11250 12000 -9750 12000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9450 12000 -7950 12000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10725 9600 -9225 9600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -8850 9600 -7350 9600
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11325 11925 -10875 11475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11925 12525 -11475 12075
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11850 12600 -10350 12600
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -9975 12600 -8475 12600
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -7725 11925 -7275 11475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8325 12525 -7875 12075
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10650 11400 -9150 11400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8850 11400 -7350 11400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10800 11250 -10800 9750
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10800 9450 -10800 7950
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11400 8550 -11400 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11400 10350 -11400 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9600 8550 -9600 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9600 10350 -9600 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9000 9750 -9000 11250
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9000 7950 -9000 9450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -7800 8550 -7800 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -7800 10350 -7800 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10087 12487 -9712 12112
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9487 11887 -9112 11512
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11887 10687 -11512 10312
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11287 10087 -10912 9712
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -7649 10124 -7274 9749
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -8249 10724 -7874 10349
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8325 8925 -7875 8475
4 0 0 50 0 0 20 0.0000 4 195 135 13125 13275 0\001
4 0 0 50 0 0 20 0.0000 4 195 135 13125 13875 1\001
4 0 0 50 0 0 20 0.0000 4 195 135 13125 14475 2\001
4 0 0 50 0 0 20 0.0000 4 195 1305 12300 12825 Label  code\001
4 0 0 50 0 0 20 0.0000 4 240 315 4050 900 [8]\001
4 0 0 50 0 0 20 0.0000 4 240 315 10650 900 [4]\001
4 0 0 50 0 0 20 0.0000 4 240 315 -2550 900 [8]\001
4 0 0 50 0 0 20 0.0000 4 240 315 -9150 900 [8]\001
4 0 0 50 0 0 20 0.0000 4 240 450 -2625 7500 [12]\001
4 0 0 50 0 0 20 0.0000 4 240 315 10650 7425 [2]\001
4 0 0 50 0 0 20 0.0000 4 240 450 4050 7500 [12]\001
4 0 0 50 0 0 20 0.0000 4 240 450 -9225 7500 [12]\001


==> figures/complete6example <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 3300 3000 75 75 3300 3000 3300 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 4500 1800 75 75 4500 1800 4500 1875
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 5700 3000 75 75 5700 3000 5700 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 3300 4500 75 75 3300 4500 3300 4575
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 5700 4500 75 75 5700 4500 5700 4575
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 4500 5700 75 75 4500 5700 4500 5775
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 4500 1800 3300 3000
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 3300 4500 3300 3000
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 3300 4500 4500 5700
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 4500 5700 5700 4500
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 5700 3000 5700 4500
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 4500 1800 5700 3000
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 4500 5700 4500 1800
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 3300 4500 4500 1800
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 3300 4500 5700 4500
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 3375 3000 5700 4500
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 3300 4500 5700 3000
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 3300 3000 5700 3000
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 3300 3000 4500 5700
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 4500 5700 5700 3000
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 4500 1800 5700 4500
4 0 0 50 0 0 20 0.0000 4 195 135 5925 4575 3\001
4 0 0 50 0 0 20 0.0000 4 195 135 2925 3075 6\001
4 0 0 50 0 0 20 0.0000 4 195 135 2925 4575 5\001
4 0 0 50 0 0 20 0.0000 4 195 135 5925 3075 2\001
4 0 0 50 0 0 20 0.0000 4 195 135 4425 1575 1\001
4 0 0 50 0 0 20 0.0000 4 195 135 4425 6150 4\001
4 0 0 50 0 0 12 0.0000 4 135 180 5025 2175 11\001
4 0 0 50 0 0 12 0.0000 4 135 90 3900 2175 3\001
4 0 0 50 0 0 12 0.0000 4 135 90 4125 2325 5\001
4 0 0 50 0 0 12 0.0000 4 135 90 4800 2325 8\001
4 0 0 50 0 0 12 0.0000 4 135 180 4575 2550 13\001
4 0 0 50 0 0 12 0.0000 4 135 180 4200 2925 10\001
4 0 0 50 0 0 12 0.0000 4 135 90 4200 3450 9\001
4 0 0 50 0 0 12 0.0000 4 135 180 3975 3900 12\001
4 0 0 50 0 0 12 0.0000 4 135 90 4650 4725 2\001
4 0 0 50 0 0 12 0.0000 4 135 90 4050 5175 4\001
4 0 0 50 0 0 12 0.0000 4 135 90 4875 5175 1\001
4 0 0 50 0 0 12 0.0000 4 135 180 5025 5475 15\001
4 0 0 50 0 0 12 0.0000 4 135 90 3900 5475 7\001
4 0 0 50 0 0 12 0.0000 4 135 90 5775 3675 6\001
4 0 0 50 0 0 12 0.0000 4 135 180 3075 3825 14\001


==> figures/cubepicture <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 4575 3000 3150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 6375 3000 4950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3150 6600 4575 6600
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4950 6600 6375 6600
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6600 6375 6600 4950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6600 4575 6600 3150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3150 3000 4575 3000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 3000 6525 3000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4350 1800 5775 1800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6150 1800 7575 1800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 3375 7800 1950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 5175 7800 3750
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4200 3450 4200 2025
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4200 5175 4200 3750
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4425 5400 5850 5400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6225 5400 7650 5400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6750 6450 7125 6075
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7275 5925 7725 5475
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3825 6000 5175 6000
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 2550 5400 3900
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 4425 5400 5775
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5625 6000 6975 6000
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3825 2400 5175 2400
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5550 2400 6900 2400
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 2625 7200 3975
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 4350 7200 5700
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 2550 3600 3900
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 4350 3600 5700
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3750 4200 5100 4200
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5625 4200 6975 4200
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6300 3600 7650 3600
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4500 3600 5850 3600
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 1950 6000 3300
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 3750 6000 5100
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4875 6450 5250 6075
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5550 5775 5925 5400
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5512 2287 5887 1912
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4912 2812 5287 2437
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3712 4087 4087 3712
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3112 4687 3487 4312
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6787 4687 7162 4312
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7387 4012 7762 3637
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 3225 4800 4575
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 5025 4800 6375
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3225 4800 4575 4800
2 1 0 1 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5025 4800 6375 4800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7387 2287 7762 1912
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6750 2925 7125 2550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3150 2850 3525 2475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3750 2250 4125 1875
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3787 5887 4162 5512
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3150 6525 3525 6150
4 0 0 50 0 0 20 0.0000 4 195 135 2925 6675 6\001
4 0 0 50 0 0 20 0.0000 4 195 270 4650 6675 16\001
4 0 0 50 0 0 20 0.0000 4 195 270 6525 6675 20\001
4 0 0 50 0 0 20 0.0000 4 195 270 2850 4875 26\001
4 0 0 50 0 0 20 0.0000 4 195 135 4725 4875 3\001
4 0 0 50 0 0 20 0.0000 4 195 270 6450 4875 13\001
4 0 0 50 0 0 20 0.0000 4 195 270 2850 3075 10\001
4 0 0 50 0 0 20 0.0000 4 195 270 4725 3075 23\001
4 0 0 50 0 0 20 0.0000 4 195 135 6525 3075 9\001
4 0 0 50 0 0 20 0.0000 4 195 270 5325 6075 21\001
4 0 0 50 0 0 20 0.0000 4 195 135 7125 6075 4\001
4 0 0 50 0 0 20 0.0000 4 195 135 5325 2475 7\001
4 0 0 50 0 0 20 0.0000 4 195 270 7050 2475 11\001
4 0 0 50 0 0 20 0.0000 4 195 270 5250 4275 14\001
4 0 0 50 0 0 20 0.0000 4 195 135 3525 4275 1\001
4 0 0 50 0 0 20 0.0000 4 195 135 6000 5475 5\001
4 0 0 50 0 0 20 0.0000 4 195 270 4200 3675 15\001
4 0 0 50 0 0 20 0.0000 4 195 135 4125 1875 8\001
4 0 0 50 0 0 20 0.0000 4 195 270 5850 1875 12\001
4 0 0 50 0 0 20 0.0000 4 195 270 7650 1875 22\001
4 0 0 50 0 0 20 0.0000 4 195 270 7650 5475 18\001
4 0 0 50 0 0 20 0.0000 4 195 135 7725 3675 2\001
4 0 0 50 0 0 20 0.0000 4 195 270 5925 3675 25\001
4 0 0 50 0 0 20 0.0000 4 195 270 4050 5475 19\001
4 0 0 50 0 0 20 0.0000 4 195 270 7125 4275 27\001
4 0 0 50 0 0 20 0.0000 4 195 270 3450 2400 24\001
4 0 0 50 0 0 20 0.0000 4 195 270 3450 6075 17\001


==> figures/durerconstruct <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 900 600 900 1800 2100 1800 2100 600 900 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 3000 600 3000 1800 4200 1800 4200 600 3000 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 5100 600 5100 1800 6300 1800 6300 600 5100 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 7200 600 7200 1800 8400 1800 8400 600 7200 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 900 2700 900 3900 2100 3900 2100 2700 900 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 3000 2700 3000 3900 4200 3900 4200 2700 3000 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 5100 2700 5100 3900 6300 3900 6300 2700 5100 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 7200 2700 7200 3900 8400 3900 8400 2700 7200 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 1800 1200 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 900 2100 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 1200 2100 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 1500 2100 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 900 4200 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 1200 4200 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 1500 4200 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 900 6300 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 1200 6300 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 1500 6300 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 1200 8400 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 1500 8400 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 3000 8400 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 3300 8400 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 3600 8400 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 3000 6300 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 3300 6300 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 3600 6300 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 3000 4200 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 3300 4200 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 3600 4200 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 3000 2100 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 3300 2100 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 3600 2100 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 900 8400 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1500 1800 1500 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1800 1800 1800 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 1800 3300 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 1800 3600 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3900 1800 3900 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 1800 5400 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5700 1800 5700 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 1800 6000 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7500 1800 7500 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 1800 7800 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8100 1800 8100 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 3900 1200 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1500 3900 1500 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1800 3900 1800 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 3900 3300 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 3900 3600 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3900 3900 3900 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 3900 5400 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5700 3900 5700 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 3900 6000 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7500 3900 7500 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 3900 7800 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8100 3900 8100 2700
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 825 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1080 3075 1125 0      0    1     0 \001
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 1425 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 1725 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 7275 825 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 7275 1125 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1080 7275 1425 0      0    1     0 \001
4 0 0 50 0 0 12 0.0000 4 135 1035 7275 1725 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 975 2925 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 975 3225 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 975 3525 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1080 975 3825 0      0    1     0 \001
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 2925 0      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 3225 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 3525 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1080 3075 3825 0      0    1     0 \001
4 0 0 50 0 0 12 0.0000 4 135 1035 5175 2925 0      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1080 5175 3225 0      0    1     0 \001
4 0 0 50 0 0 12 0.0000 4 135 1035 5175 3525 1      0    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 5175 3825 0      0    0     1\001
4 0 0 50 0 0 18 0.0000 4 45 150 6675 3375 =\001
4 0 0 50 0 0 12 0.0000 4 135 990 975 825 0     0     1    0\001
4 0 0 50 0 0 12 0.0000 4 135 990 975 1125 0     1     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 975 1425 0     0     0     1\001
4 0 0 50 0 0 12 0.0000 4 135 990 975 1725 1     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 5175 825 0     0     0     1\001
4 0 0 50 0 0 12 0.0000 4 135 990 5175 1125 1     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 990 5175 1425 0     0     1    0\001
4 0 0 50 0 0 12 0.0000 4 135 990 5175 1725 0     1     0    0\001
4 0 0 50 0 0 20 0.0000 4 195 285 2475 3375 +8\001
4 0 0 50 0 0 20 0.0000 4 195 135 525 1275 2\001
4 0 0 50 0 0 20 0.0000 4 195 420 2400 1275 +10\001
4 0 0 50 0 0 20 0.0000 4 195 285 4500 1275 +5\001
4 0 0 50 0 0 20 0.0000 4 195 285 6675 1275 +2\001
4 0 0 50 0 0 20 0.0000 4 195 285 450 3375 +6\001
4 0 0 50 0 0 20 0.0000 4 135 150 4575 3375 +\001
4 0 0 50 0 0 12 0.0000 4 135 1080 7275 2925 16    3    2    13\001
4 0 0 50 0 0 12 0.0000 4 135 1035 7275 3225 5     10   11   8\001
4 0 0 50 0 0 12 0.0000 4 135 1080 7275 3525 9     6      7   12\001
4 0 0 50 0 0 12 0.0000 4 135 1035 7275 3825  4   15   14    1\001


==> figures/evenmagicconstruct <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 1200 1800 1200 4200 3600 4200 3600 1800 1200 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1800 1800 1800 4200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 2400 3600 2400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 3000 3600 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 3600 3600 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 1800 2400 4200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 1800 3000 4200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 6000 1800 6000 4200 8400 4200 8400 1800 6000 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 2400 8400 2400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 3000 8400 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 3600 8400 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1800 1800 1800 4200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6600 1800 6600 4200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 1800 7200 4200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 1800 7800 4200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 3900 3000 5475 3000
4 0 0 50 0 0 20 0.0000 4 195 135 3225 2175 4\001
4 0 0 50 0 0 20 0.0000 4 195 270 1950 3375 10\001
4 0 0 50 0 0 20 0.0000 4 195 270 2625 3375 11\001
4 0 0 50 0 0 12 0.0000 4 135 675 2025 2175 2           3\001
4 0 0 50 0 0 20 0.0000 4 195 135 1425 2175 1\001
4 0 0 50 0 0 12 0.0000 4 135 90 1425 2775 5\001
4 0 0 50 0 0 20 0.0000 4 195 135 2025 2850 6\001
4 0 0 50 0 0 20 0.0000 4 195 135 2625 2850 7\001
4 0 0 50 0 0 12 0.0000 4 135 90 3225 2775 8\001
4 0 0 50 0 0 12 0.0000 4 135 90 1425 3375 9\001
4 0 0 50 0 0 12 0.0000 4 135 180 3225 3375 12\001
4 0 0 50 0 0 12 0.0000 4 135 810 1950 3975 14          15\001
4 0 0 50 0 0 20 0.0000 4 195 270 3150 3975 16\001
4 0 0 50 0 0 20 0.0000 4 195 270 1350 3975 13\001
4 0 0 50 0 0 20 0.0000 4 195 135 6225 2175 1\001
4 0 0 50 0 0 20 0.0000 4 195 135 8025 2175 4\001
4 0 0 50 0 0 20 0.0000 4 195 135 6825 2775 6\001
4 0 0 50 0 0 20 0.0000 4 195 135 7425 2775 7\001
4 0 0 50 0 0 20 0.0000 4 195 270 6750 3375 10\001
4 0 0 50 0 0 20 0.0000 4 195 270 7350 3375 11\001
4 0 0 50 0 0 12 0.0000 4 135 765 6825 2175 15         14\001
4 0 0 50 0 0 12 0.0000 4 135 1890 6150 2775  12                                   9\001
4 0 0 50 0 0 12 0.0000 4 135 135 6150 3375  8\001
4 0 0 50 0 0 12 0.0000 4 135 90 8025 3375 5\001
4 0 0 50 0 0 12 0.0000 4 135 765 6825 3975 3             2\001
4 0 0 50 0 0 20 0.0000 4 195 270 6150 3975 13\001
4 0 0 50 0 0 20 0.0000 4 195 270 7950 3975 16\001


==> figures/hagstorm <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 300 3300 300 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 300 900 2700 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 300 1200 2700 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 300 1500 2700 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 300 1800 2700 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 300 2100 2700 2100
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 300 2400 2700 2400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 300 2700 2700 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 300 3000 2700 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 300 3300 2700 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 3300 600 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 3300 900 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 3300 1200 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1500 3300 1500 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1800 3300 1800 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2100 3300 2100 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 3300 2400 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 3300 2700 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 900 5700 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6300 900 8700 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 3300 3300 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 3300 3600 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3900 3300 3900 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4200 3300 4200 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4500 3300 4500 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 3300 4800 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 3300 5100 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 3300 5400 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5700 3300 5700 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 1200 5700 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 1500 5700 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 1800 5700 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 2100 5700 2100
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 2400 5700 2400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 2700 5700 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 3000 5700 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 3300 5700 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6300 3300 6300 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6600 3300 6600 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 3300 6900 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 3300 7200 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7500 3300 7500 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 3300 7800 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8100 3300 8100 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8400 3300 8400 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8700 3300 8700 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6300 1200 8700 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6300 1500 8700 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6300 1800 8700 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6300 2100 8700 2100
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6300 2400 8700 2400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6300 2700 8700 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6300 3000 8700 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6300 3300 8700 3300
4 0 0 50 0 0 12 0.0000 4 135 2340 300 1125  30   55  12   33   14   49  28   39\001
4 0 0 50 0 0 12 0.0000 4 135 2340 300 1425  11   34  29   56   27   40  13   50\001
4 0 0 50 0 0 12 0.0000 4 135 2340 300 1725  53   32   35  10   37  26   51   16\001
4 0 0 50 0 0 12 0.0000 4 135 2340 300 2025  36    9   54   31   52  15   38   25\001
4 0 0 50 0 0 12 0.0000 4 135 2340 300 2325  22   63    4   41    6    57  20   47\001
4 0 0 50 0 0 12 0.0000 4 135 2340 300 2625  44    1   62   23   60    7   46   17\001
4 0 0 50 0 0 12 0.0000 4 135 2295 300 2925  61   24   43   2    45   18  59    8\001
4 0 0 50 0 0 12 0.0000 4 135 2250 375 3225 3    42   21   64  19   48    5   58\001
4 0 0 50 0 0 12 0.0000 4 135 2340 3300 1125  44   19   45  22   41  18   48   23\001
4 0 0 50 0 0 12 0.0000 4 135 2340 3300 1425  13   54  12   51   16   55   9    50\001
4 0 0 50 0 0 12 0.0000 4 135 2340 3300 1725  20   43   21  46   17   42  24   47\001
4 0 0 50 0 0 12 0.0000 4 135 2340 3300 2025  53   14   52  11   56  15   49   10\001
4 0 0 50 0 0 12 0.0000 4 135 2430 3300 2325   4    59    5   62    1    58   8    63  \001
4 0 0 50 0 0 12 0.0000 4 135 2295 3300 2925  60    3    61   6    57    2   64    7\001
4 0 0 50 0 0 12 0.0000 4 135 2340 3300 2625  29   38  28   35   32   39  25   34\001
4 0 0 50 0 0 12 0.0000 4 135 2340 3300 3225  37   30   36  27   40   31  33   26\001
4 0 0 50 0 0 12 0.0000 4 135 2430 6300 1125  37   60  23   10   39   58  21   12  \001
4 0 0 50 0 0 12 0.0000 4 135 2340 6300 1425  24    9    38  59   22   11  40   57\001
4 0 0 50 0 0 12 0.0000 4 135 2295 6300 1725  42   55   28   5    44  53   26    7\001
4 0 0 50 0 0 12 0.0000 4 135 2340 6300 2025  27    6   41   56   25    8    43  54\001
4 0 0 50 0 0 12 0.0000 4 135 2340 6300 2325  46   51   32   1    48   49  30    3 \001
4 0 0 50 0 0 12 0.0000 4 135 2520 6300 2625  31    2   45   52   29   4    47   50    \001
4 0 0 50 0 0 12 0.0000 4 135 2340 6300 2925  33   64  19   14   35   62  17   16\001
4 0 0 50 0 0 12 0.0000 4 135 2340 6300 3225  20   13   34  63   18  15   36   61\001


==> figures/irreducible <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 2100 2700 84 84 2025 2663 2175 2738
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 3300 2700 84 84 3225 2663 3375 2738
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 3300 3600 84 84 3225 3563 3375 3638
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 2100 3600 84 84 2025 3563 2175 3638
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 5100 2709 84 84 5025 2672 5175 2747
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 5100 3600 84 84 5025 3563 5175 3638
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 6300 3600 84 84 6225 3563 6375 3638
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 6300 2700 84 84 6225 2663 6375 2738
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 7800 2700 84 84 7725 2663 7875 2738
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 9000 3609 84 84 8925 3572 9075 3647
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 9000 2709 84 84 8925 2672 9075 2747
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 7800 3600 84 84 7725 3563 7875 3638
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2100 2700 3225 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2100 2700 2100 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2175 3600 3300 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 2700 6225 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 2775 9000 3675
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 2700 3300 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 2775 7800 3675
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 5100 3600 5100 2700
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 6300 3600 6300 2700
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 7800 2700 9000 2700
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 9075 3600 7800 3600
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 10350 2925 10350 4050 12375 4050 12375 2925 10350 2925
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 10500 3450 11100 3450
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 10500 3750 11100 3750
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5175 3600 6300 3600
4 0 0 50 0 0 30 0.0000 4 90 210 4125 3375 =\001
4 0 0 50 0 0 30 0.0000 4 180 210 6975 3375 +\001
4 0 0 50 0 0 12 0.0000 4 180 390 10500 3225 Edge\001
4 0 0 50 0 0 12 0.0000 4 135 420 11625 3225 Label\001
4 0 0 50 0 0 12 0.0000 4 135 90 11775 3825 1\001
4 0 0 50 0 0 12 0.0000 4 135 90 11775 3525 0\001


==> figures/konigscayley <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 5700 4800 75 75 5700 4800 5700 4875
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 4800 3900 75 75 4800 3900 4800 3975
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 3900 4800 75 75 3900 4800 3900 4875
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 4800 1800 75 75 4800 1800 4800 1875
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 2400 5700 75 75 2400 5700 2400 5775
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 7200 5700 75 75 7200 5700 7200 5775
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 4806 4522 2730 2730 4806 4522 5781 7072
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 2400 5700 3000 5100 3825 4875
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 3900 4875 3300 5400 2475 5625
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 5775 4875 6300 5400 7050 5700
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 7125 5625 6600 5100 5850 4875
	 0.000 -1.000 0.000
3 0 0 1 0 7 50 0 -1 0.000 0 1 0 2
	1 1 1.00 60.00 120.00
	 3300 2250 3375 2175
	 0.000 0.000
3 0 0 1 0 7 50 0 -1 0.000 0 1 0 2
	1 1 1.00 60.00 120.00
	 7275 3300 7350 3525
	 0.000 0.000
3 0 0 1 0 7 50 0 -1 0.000 0 1 0 2
	1 1 1.00 60.00 120.00
	 5100 7200 4875 7275
	 0.000 0.000
3 0 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 3900 4800 4200 4200 4725 3900
	 0.000 1.000 0.000
3 0 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 4800 3975 4500 4500 3975 4800
	 0.000 1.000 0.000
3 0 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 4875 3900 5400 4200 5700 4725
	 0.000 1.000 0.000
3 0 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 5625 4800 5100 4500 4875 3975
	 0.000 1.000 0.000
3 0 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 3975 4875 4800 5100 5625 4875
	 0.000 1.000 0.000
3 0 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 5550 4800 4800 4650 3975 4875
	 0.000 1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 4725 1800 3600 3900 3900 4650
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 3825 4800 3000 4200 4650 1800
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 4875 1875 6000 3900 5775 4650
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 5850 4800 6600 3900 4950 1800
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 3900 4875 5700 6300 7200 5775
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 7050 5775 5925 6000 4050 4950
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 5700 4875 3900 6300 2475 5775
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 2475 5700 3600 6075 5475 5025
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 4800 3900 3000 3900 2400 5550
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 2400 5550 3300 4200 4575 3900
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 4875 3900 6675 3900 7275 5550
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 7200 5550 6450 4125 5025 3900
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 4725 1800 2775 3600 2325 5550
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 7200 5700 7200 3900 5025 1800
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 2400 5775 4800 6900 7050 6000
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 4833 3816 4533 2691 4758 1866
	 0.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 1 0 3
	1 1 1.00 60.00 120.00
	 4811 1893 5111 2718 4886 3843
	 0.000 -1.000 0.000
4 0 0 50 0 0 12 0.0000 4 135 90 5475 4275 1\001
4 0 0 50 0 0 12 0.0000 4 135 90 5100 4350 2\001
4 0 0 50 0 0 12 0.0000 4 135 90 4125 4275 4\001
4 0 0 50 0 0 12 0.0000 4 135 90 4425 4425 4\001
4 0 0 50 0 0 12 0.0000 4 135 90 4575 2700 5\001
4 0 0 50 0 0 12 0.0000 4 135 90 7200 4650 3\001
4 0 0 50 0 0 12 0.0000 4 135 90 6975 4800 3\001
4 0 0 50 0 0 12 0.0000 4 135 90 2550 4725 1\001
4 0 0 50 0 0 12 0.0000 4 135 90 2850 4950 2\001
4 0 0 50 0 0 12 0.0000 4 135 90 4725 4650 5\001
4 0 0 50 0 0 12 0.0000 4 135 90 4875 5025 5\001
4 0 0 50 0 0 12 0.0000 4 135 90 5850 3000 3\001
4 0 0 50 0 0 12 0.0000 4 135 90 5550 3225 3\001
4 0 0 50 0 0 12 0.0000 4 135 90 6600 5025 4\001
4 0 0 50 0 0 12 0.0000 4 135 90 6450 5475 4\001
4 0 0 50 0 0 12 0.0000 4 135 90 4200 6075 1\001
4 0 0 50 0 0 12 0.0000 4 135 90 3750 6000 2\001
4 0 0 50 0 0 12 0.0000 4 135 90 3525 3300 1\001
4 0 0 50 0 0 12 0.0000 4 135 90 3975 3300 2\001
4 0 0 50 0 0 12 0.0000 4 135 90 5475 6225 2\001
4 0 0 50 0 0 12 0.0000 4 135 90 6075 6000 1\001
4 0 0 50 0 0 12 0.0000 4 135 90 7200 3075 1\001
4 0 0 50 0 0 12 0.0000 4 135 90 6825 3300 2\001
4 0 0 50 0 0 12 0.0000 4 135 90 3450 2625 4\001
4 0 0 50 0 0 12 0.0000 4 135 90 2775 2625 4\001
4 0 0 50 0 0 12 0.0000 4 135 90 4800 6825 5\001
4 0 0 50 0 0 12 0.0000 4 135 90 4875 7200 5\001
4 0 0 50 0 0 12 0.0000 4 135 90 5025 2700 5\001
4 0 0 50 0 0 12 0.0000 4 135 90 2925 5325 3\001
4 0 0 50 0 0 12 0.0000 4 135 90 3075 5700 3\001
4 0 0 50 0 0 24 0.0000 4 255 180 5625 5325 2\001
4 0 0 50 0 0 24 0.0000 4 255 180 3825 5325 3\001
4 0 0 50 0 0 24 0.0000 4 255 180 4725 1650 4\001
4 0 0 50 0 0 24 0.0000 4 255 180 7350 5850 5\001
4 0 0 50 0 0 24 0.0000 4 255 180 2025 5925 6\001
4 0 0 50 0 0 24 0.0000 4 255 180 4800 3675 1\001


==> figures/magiccubeconstruct <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -11925 5925 150 150 -11925 5925 -11775 5925
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -8400 2400 150 150 -8400 2400 -8250 2400
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -11994 2442 150 150 -11994 2442 -11994 2592
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -8394 5967 150 150 -8394 5967 -8394 6117
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -7200 4800 150 150 -7200 4800 -7050 4800
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -10725 1275 150 150 -10725 1275 -10575 1275
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -7275 1275 150 150 -7275 1275 -7275 1425
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -10800 4800 150 150 -10800 4800 -10800 4950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 6031 13244 150 150 6031 13244 6031 13394
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 6000 14400 150 150 6000 14400 6150 14400
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -5400 4200 150 150 -5400 4200 -5250 4200
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -3600 2400 150 150 -3600 2400 -3450 2400
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -3600 4200 150 150 -3600 4200 -3600 4350
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -5325 2400 150 150 -5325 2400 -5325 2550
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -3000 5400 150 150 -3000 5400 -2850 5400
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -1200 3600 150 150 -1200 3600 -1050 3600
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -4800 1800 150 150 -4800 1800 -4650 1800
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -2956 1831 150 150 -2956 1831 -2956 1981
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -4756 3631 150 150 -4756 3631 -4756 3781
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -1231 5356 150 150 -1231 5356 -1231 5506
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -2400 4800 150 150 -2400 4800 -2400 4950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -600 3000 150 150 -600 3000 -600 3150
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -600 4800 150 150 -600 4800 -450 4800
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -2400 3000 150 150 -2400 3000 -2250 3000
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 1200 5925 150 150 1200 5925 1200 6075
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 3000 4200 150 150 3000 4200 3000 4350
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 4800 2400 150 150 4800 2400 4800 2550
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 4800 6000 150 150 4800 6000 4950 6000
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 1200 4200 150 150 1200 4200 1350 4200
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 3000 2400 150 150 3000 2400 3150 2400
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 3600 5400 150 150 3600 5400 3750 5400
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 5400 3600 150 150 5400 3600 5550 3600
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 1800 1800 150 150 1800 1800 1950 1800
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 5400 5400 150 150 5400 5400 5400 5550
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 3600 1800 150 150 3600 1800 3600 1950
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 2400 4800 150 150 2400 4800 2550 4800
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 4200 3000 150 150 4200 3000 4350 3000
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 5925 1275 150 150 5925 1275 6075 1275
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 4200 4800 150 150 4200 4800 4200 4950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 6000 3000 150 150 6000 3000 6000 3150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 2400 1275 150 150 2400 1275 2400 1425
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 1800 3600 150 150 1800 3600 1800 3750
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -12000 12600 150 150 -12000 12600 -12000 12750
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -10125 12600 150 150 -10125 12600 -9975 12600
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -12000 10800 150 150 -12000 10800 -11850 10800
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -10200 10800 150 150 -10200 10800 -10200 10950
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -11400 12000 150 150 -11400 12000 -11250 12000
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -7800 10200 150 150 -7800 10200 -7650 10200
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -9600 8400 150 150 -9600 8400 -9450 8400
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -9600 12000 150 150 -9600 12000 -9600 12150
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -11400 10200 150 150 -11400 10200 -11400 10350
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -7800 8400 150 150 -7800 8400 -7800 8550
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -9000 9600 150 150 -9000 9600 -8850 9600
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -7200 7875 150 150 -7200 7875 -7050 7875
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -9000 7800 150 150 -9000 7800 -9000 7950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -7200 9600 150 150 -7200 9600 -7200 9750
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -5356 12569 150 150 -5356 12569 -5356 12719
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -1800 10800 150 150 -1800 10800 -1800 10950
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -1800 12600 150 150 -1800 12600 -1650 12600
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -3600 10800 150 150 -3600 10800 -3450 10800
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -5400 9000 150 150 -5400 9000 -5250 9000
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -3600 9000 150 150 -3600 9000 -3600 9150
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -4831 12031 150 150 -4831 12031 -4681 12031
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -1200 10200 150 150 -1200 10200 -1050 10200
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -3000 8400 150 150 -3000 8400 -2850 8400
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -1200 8400 150 150 -1200 8400 -1200 8550
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -4800 10200 150 150 -4800 10200 -4800 10350
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -3000 12000 150 150 -3000 12000 -3000 12150
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -2400 11400 150 150 -2400 11400 -2250 11400
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -4200 9600 150 150 -4200 9600 -4050 9600
1 3 0 1 19 19 50 0 41 0.000 1 0.0000 -675 7875 150 150 -675 7875 -525 7875
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -4200 7800 150 150 -4200 7800 -4200 7950
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -2400 9600 150 150 -2400 9600 -2400 9750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 6000 4800 150 150 6000 4800 6000 4950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 3075 6000 150 150 3075 6000 3075 6150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 1800 5400 150 150 1800 5400 1800 5550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 1200 2400 150 150 1200 2400 1200 2550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 4200 1200 150 150 4200 1200 4200 1350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 5400 1800 150 150 5400 1800 5400 1950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 2400 3000 150 150 2400 3000 2400 3150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 3600 3600 150 150 3600 3600 3600 3750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 4800 4200 150 150 4800 4200 4800 4350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -4200 1200 150 150 -4200 1200 -4200 1350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -2400 1200 150 150 -2400 1200 -2400 1350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -1800 2400 150 150 -1800 2400 -1800 2550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -1275 1800 150 150 -1275 1800 -1275 1950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -675 1275 150 150 -675 1275 -675 1425
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -4200 3000 150 150 -4200 3000 -4200 3150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -4200 4800 150 150 -4200 4800 -4200 4950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -4800 5400 150 150 -4800 5400 -4800 5550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -5400 5925 150 150 -5400 5925 -5400 6075
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -3600 6000 150 150 -3600 6000 -3600 6150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -3000 3600 150 150 -3000 3600 -3000 3750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -1800 4200 150 150 -1800 4200 -1800 4350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -1800 6000 150 150 -1800 6000 -1800 6150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -7800 5400 150 150 -7800 5400 -7800 5550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -8400 4200 150 150 -8400 4200 -8400 4350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -7800 3600 150 150 -7800 3600 -7800 3750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -7200 3000 150 150 -7200 3000 -7200 3150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -7800 1725 150 150 -7800 1725 -7800 1875
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -9000 1200 150 150 -9000 1200 -9000 1350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -9600 1800 150 150 -9600 1800 -9600 1950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -10200 2400 150 150 -10200 2400 -10200 2550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -11400 1800 150 150 -11400 1800 -11400 1950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -12000 4200 150 150 -12000 4200 -12000 4350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -11400 3600 150 150 -11400 3600 -11400 3750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -10800 3000 150 150 -10800 3000 -10800 3150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -9000 3000 150 150 -9000 3000 -9000 3150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -9600 3600 150 150 -9600 3600 -9600 3750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -10200 4200 150 150 -10200 4200 -10200 4350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -11400 5400 150 150 -11400 5400 -11400 5550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -10200 6000 150 150 -10200 6000 -10200 6150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -9525 5400 150 150 -9525 5400 -9525 5550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -9000 4800 150 150 -9000 4800 -9000 4950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -10800 7800 150 150 -10800 7800 -10800 7950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -11400 8400 150 150 -11400 8400 -11400 8550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -11925 9000 150 150 -11925 9000 -11925 9150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -10200 9000 150 150 -10200 9000 -10200 9150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -8400 9000 150 150 -8400 9000 -8400 9150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -10800 9600 150 150 -10800 9600 -10800 9750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -9600 10200 150 150 -9600 10200 -9600 10350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -8400 10800 150 150 -8400 10800 -8400 10950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -9000 11400 150 150 -9000 11400 -9000 11550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -7200 11400 150 150 -7200 11400 -7200 11550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -7800 12000 150 150 -7800 12000 -7800 12150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -8400 12600 150 150 -8400 12600 -8400 12750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -10800 11400 150 150 -10800 11400 -10800 11550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -5400 10800 150 150 -5400 10800 -5400 10950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -4800 8400 150 150 -4800 8400 -4800 8550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -2400 7800 150 150 -2400 7800 -2400 7950
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -1875 9000 150 150 -1875 9000 -1875 9150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -600 9600 150 150 -600 9600 -600 9750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -3000 10200 150 150 -3000 10200 -3000 10350
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -1125 12000 150 150 -1125 12000 -1125 12150
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -3600 12600 150 150 -3600 12600 -3600 12750
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 -4125 11400 150 150 -4125 11400 -4125 11550
1 3 0 1 13 13 50 0 41 0.000 1 0.0000 -600 11400 150 150 -600 11400 -600 11550
1 3 0 1 3 3 50 0 41 0.000 1 0.0000 6000 13800 150 150 6000 13800 6000 13950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1350 6000 2850 6000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3225 6000 4650 6000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 4350 1200 5850
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 4050 1200 2550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1350 2400 2850 2400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3150 2400 4650 2400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 4050 4800 2550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 5850 4800 4350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4350 1200 5850 1200
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2550 1200 4050 1200
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5550 1650 5925 1275
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4875 2250 5250 1875
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 4650 2400 3150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1275 5850 1650 5475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1875 5250 2325 4800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2550 4800 4050 4800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4350 4800 5850 4800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5550 5325 6000 4875
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4950 5925 5325 5550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 2850 6000 1350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 4650 6000 3150
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5400 3450 5400 2025
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5400 5175 5400 3750
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5550 3525 5925 3150
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1350 4050 1725 3675
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1950 3450 2325 3075
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1800 3375 1800 1950
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1800 5175 1800 3750
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1950 5400 3450 5400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3750 5400 5250 5400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3150 5850 3525 5475
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4950 4050 5325 3675
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4200 2775 4200 1350
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4200 4575 4200 3150
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 2550 3000 4050 3000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4350 3000 5850 3000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3750 1800 5250 1800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1950 3600 3450 3600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1950 3600 3450 3600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3750 3600 5250 3600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3600 3375 3600 1950
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3600 5175 3600 3750
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1350 4200 2850 4200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3150 4200 4650 4200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3000 3975 3000 2550
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3000 5775 3000 4350
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3075 2250 3450 1875
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3712 1687 4087 1312
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1312 2287 1687 1912
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1912 1687 2287 1312
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 11250 6000 9750
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 9450 2400 7950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 11250 2400 9750
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2550 7800 4050 7800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4350 7800 5850 7800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4350 11400 5850 11400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2550 11400 4050 11400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3150 12600 4650 12600
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1350 12600 2850 12600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3150 12525 3525 12150
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3750 11925 4125 11550
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4200 9750 4200 11250
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4200 7875 4200 9375
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1950 12000 3450 12000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 12450 4800 10950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 12450 1200 10950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 10650 4800 9150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 10650 1200 9150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1350 9000 2850 9000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3675 8250 4050 7875
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3075 8850 3450 8475
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1950 8400 3450 8400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3750 8400 5250 8400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5400 8550 5400 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5400 10350 5400 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4912 10687 5287 10312
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5512 10087 5887 9712
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1800 8550 1800 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1800 10350 1800 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1350 10800 2850 10800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3150 10800 4650 10800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3000 9150 3000 10650
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3000 10950 3000 12450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3600 8550 3600 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3600 10350 3600 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 2550 9600 4050 9600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4350 9600 5850 9600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1312 10687 1687 10312
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1912 10087 2287 9712
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1950 1800 3450 1800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 2850 2400 1350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -600 2850 -600 1350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5250 6000 -3750 6000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -3450 6000 -1950 6000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5400 5850 -5400 4350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5400 4050 -5400 2550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1800 4050 -1800 2550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1800 5850 -1800 4350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5250 2400 -3750 2400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4050 4800 -2550 4800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -2250 4800 -750 4800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5325 5850 -4950 5475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4050 1200 -2550 1200
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -2250 1200 -750 1200
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4725 1650 -4350 1275
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5325 2250 -4950 1875
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4200 2850 -4200 1350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4200 4650 -4200 3150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4687 5212 -4312 4837
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1687 5887 -1312 5512
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1087 5287 -712 4912
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1724 2249 -1349 1874
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -5250 4200 -3750 4200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3450 4200 -1950 4200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3000 5175 -3000 3750
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -1200 1950 -1200 3450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -1200 3750 -1200 5250
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4800 1950 -4800 3450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4800 3750 -4800 5250
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4650 5400 -3150 5400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2850 5400 -1350 5400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4650 1800 -3150 1800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2850 1800 -1350 1800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -5288 4087 -4913 3712
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4687 3487 -4312 3112
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -1687 4087 -1312 3712
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -1012 3487 -637 3112
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2887 5287 -2512 4912
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3487 5887 -3112 5512
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2887 1687 -2512 1312
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4050 3000 -2550 3000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2250 3000 -750 3000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2400 4575 -2400 3150
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2400 2775 -2400 1350
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4650 3600 -3150 3600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2850 3600 -1350 3600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3600 3975 -3600 2550
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3600 5775 -3600 4350
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3000 3375 -3000 1950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -3450 2400 -1950 2400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3524 2249 -3149 1874
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10650 1200 -9150 1200
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8850 1200 -7350 1200
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8850 4800 -7350 4800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10650 4800 -9150 4800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -7200 4650 -7200 3150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -7200 2850 -7200 1350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10800 2850 -10800 1350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10800 4650 -10800 3150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11850 6000 -10350 6000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10050 6000 -8550 6000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11850 2400 -10350 2400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10050 2400 -8550 2400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8400 4050 -8400 2550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8400 5850 -8400 4350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -12000 4050 -12000 2550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -12000 5850 -12000 4350
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8287 5887 -7912 5512
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -7687 5287 -7312 4912
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11287 5287 -10912 4912
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11887 5887 -11512 5512
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11887 2287 -11512 1912
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11287 1687 -10912 1312
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8324 2249 -7949 1874
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -7724 1649 -7349 1274
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10124 2249 -9749 1874
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9524 1649 -9149 1274
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11924 4049 -11549 3674
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11324 3449 -10949 3074
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -7724 3449 -7349 3074
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10049 5849 -9674 5474
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9449 5249 -9074 4874
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -8286 4086 -7911 3711
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11250 3600 -9750 3600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9450 3600 -7950 3600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11250 1800 -9750 1800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9450 1800 -7950 1800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11250 5400 -9750 5400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9450 5400 -7950 5400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9600 3750 -9600 5250
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11400 1950 -11400 3450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -7800 1950 -7800 3450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -7800 3750 -7800 5250
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11400 3750 -11400 5250
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10200 2550 -10200 4050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10200 4350 -10200 5850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11850 4200 -10350 4200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10050 4200 -8550 4200
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4050 7800 -2550 7800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -2250 7800 -750 7800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -600 9450 -600 7950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -600 11250 -600 9750
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4200 9450 -4200 7950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4050 11400 -2550 11400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -2250 11400 -750 11400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5250 9000 -3750 9000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -3450 12600 -1950 12600
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5250 12600 -3750 12600
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5400 10650 -5400 9150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5400 12450 -5400 10950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1800 10650 -1800 9150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1800 12450 -1800 10950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5325 8850 -4875 8400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4725 8250 -4275 7800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -5325 12525 -4875 12075
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4725 11925 -4275 11475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1725 8925 -1275 8475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1125 8325 -675 7875
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4650 8400 -3150 8400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2925 8400 -1425 8400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2850 10200 -1350 10200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2850 12000 -1350 12000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4650 12000 -3150 12000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4650 10200 -3150 10200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3000 8550 -3000 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3000 10350 -3000 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2400 7950 -2400 9450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2400 9675 -2400 11175
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4800 8550 -4800 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4800 10350 -4800 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -1200 8550 -1200 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -1200 10350 -1200 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3488 12487 -3113 12112
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2887 11887 -2512 11512
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -1687 10687 -1312 10312
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -1087 10087 -712 9712
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -5287 10687 -4912 10312
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4687 10087 -4312 9712
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3487 8887 -3112 8512
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2887 8287 -2512 7912
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -4050 9600 -2550 9600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -2250 9600 -750 9600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3600 10950 -3600 12450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3600 9150 -3600 10650
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -5250 10800 -3750 10800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -3450 10800 -1950 10800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10650 7800 -9150 7800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8850 7800 -7350 7800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10050 9000 -8550 9000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11850 9000 -10350 9000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11962 8887 -11512 8437
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11362 8287 -10912 7837
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -7687 8362 -7237 7912
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11250 8400 -9750 8400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9450 8400 -7950 8400
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9524 8249 -9149 7874
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10124 8849 -9749 8474
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8400 10650 -8400 9150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -7200 9450 -7200 7950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -7200 11250 -7200 9750
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8400 12450 -8400 10950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -12000 10650 -12000 9150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -12000 12450 -12000 10950
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11850 10800 -10350 10800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10050 10800 -8550 10800
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10200 9150 -10200 10650
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10200 10950 -10200 12450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11250 10200 -9750 10200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9450 10200 -7950 10200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11250 12000 -9750 12000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9450 12000 -7950 12000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10725 9600 -9225 9600
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -8850 9600 -7350 9600
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11325 11925 -10875 11475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11925 12525 -11475 12075
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -11850 12600 -10350 12600
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -9975 12600 -8475 12600
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -7725 11925 -7275 11475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8325 12525 -7875 12075
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10650 11400 -9150 11400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8850 11400 -7350 11400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10800 11250 -10800 9750
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -10800 9450 -10800 7950
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11400 8550 -11400 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11400 10350 -11400 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9600 8550 -9600 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9600 10350 -9600 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9000 9750 -9000 11250
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9000 7950 -9000 9450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -7800 8550 -7800 10050
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -7800 10350 -7800 11850
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10087 12487 -9712 12112
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9487 11887 -9112 11512
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11887 10687 -11512 10312
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -11287 10087 -10912 9712
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -7649 10124 -7274 9749
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -8249 10724 -7874 10349
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -8325 8925 -7875 8475
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9600 1950 -9600 3450
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -10650 3000 -9150 3000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -8850 3000 -7350 3000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9000 2775 -9000 1350
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 -9000 4650 -9000 3225
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -600 4650 -600 3150
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3712 5287 4087 4912
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -3525 9000 -2025 9000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1650 12525 -1200 12075
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1050 11925 -600 11475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -4200 11250 -4200 9750
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3150 9000 4650 9000
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3750 12000 5250 12000
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5550 8250 5850 7950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 9450 6000 7950
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4875 8850 5250 8475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5550 11850 5850 11550
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4950 12450 5250 12150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1275 12450 1575 12150
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1950 11775 2250 11475
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1875 8175 2250 7800
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 8850 1650 8400
2 1 0 3 24 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1124 1724 -749 1349
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1875 10200 3375 10200
2 1 0 1 24 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3750 10200 5250 10200
4 0 0 50 0 0 24 0.0000 4 255 480 -6675 3675 + 4\001
4 0 0 50 0 0 20 0.0000 4 195 135 6525 14475 2\001
4 0 0 50 0 0 20 0.0000 4 195 135 6525 13875 1\001
4 0 0 50 0 0 20 0.0000 4 195 135 6525 13350 0\001
4 0 0 50 0 0 20 0.0000 4 195 1245 5700 12900 Label  code\001
4 0 0 50 0 0 24 0.0000 4 255 480 150 3750 + 6\001
4 0 0 50 0 0 24 0.0000 4 255 570 -13050 10275 +  2\001
4 0 0 50 0 0 24 0.0000 4 180 210 -6375 10275 +\001
4 0 0 50 0 0 24 0.0000 4 90 210 225 10050 =\001
4 0 0 50 0 0 20 0.0000 4 195 135 1125 12675 6\001
4 0 0 50 0 0 20 0.0000 4 195 270 2850 12675 16\001
4 0 0 50 0 0 20 0.0000 4 195 270 4650 12675 20\001
4 0 0 50 0 0 20 0.0000 4 195 270 1125 10875 26\001
4 0 0 50 0 0 20 0.0000 4 195 135 2925 10875 3\001
4 0 0 50 0 0 20 0.0000 4 195 270 4650 10875 13\001
4 0 0 50 0 0 20 0.0000 4 195 270 1050 9075 10\001
4 0 0 50 0 0 20 0.0000 4 195 270 2850 9075 23\001
4 0 0 50 0 0 20 0.0000 4 195 135 4725 9075 9\001
4 0 0 50 0 0 20 0.0000 4 195 270 1650 12075 17\001
4 0 0 50 0 0 20 0.0000 4 195 270 3450 12075 21\001
4 0 0 50 0 0 20 0.0000 4 195 135 5325 12075 4\001
4 0 0 50 0 0 20 0.0000 4 195 135 1725 10275 1\001
4 0 0 50 0 0 20 0.0000 4 195 270 3450 10275 14\001
4 0 0 50 0 0 20 0.0000 4 195 270 5250 10275 27\001
4 0 0 50 0 0 20 0.0000 4 195 135 3525 8475 7\001
4 0 0 50 0 0 20 0.0000 4 195 135 4125 11475 5\001
4 0 0 50 0 0 20 0.0000 4 195 270 5925 11475 18\001
4 0 0 50 0 0 20 0.0000 4 195 270 4125 9675 25\001
4 0 0 50 0 0 20 0.0000 4 195 135 2325 7875 8\001
4 0 0 50 0 0 20 0.0000 4 195 270 4050 7875 12\001
4 0 0 50 0 0 20 0.0000 4 195 270 5250 8400 11\001
4 0 0 50 0 0 20 0.0000 4 195 270 5850 7875 22\001
4 0 0 50 0 0 20 0.0000 4 195 135 5925 9675 2\001
4 0 0 50 0 0 20 0.0000 4 195 270 2250 11475 19\001
4 0 0 50 0 0 20 0.0000 4 195 270 2250 9675 15\001
4 0 0 50 0 0 20 0.0000 4 195 270 1650 8400 24\001


==> figures/magiccubehbasis <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 4
	 2400 4800 3300 3900 4200 3000 4200 3075
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3600 2400 3600 4875
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 5
	 2400 2400 2400 4800 4800 4800 4800 2400 2400 2400
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 2400 3600 4800 3600
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 5
	 3375 1500 3375 3900 5775 3900 5775 1500 3375 1500
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 5
	 4200 600 4200 3000 6600 3000 6600 600 4200 600
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4200 600 2400 2400
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3675 2400 5400 600
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4800 2400 6600 600
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4800 4800 6675 3000
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3600 4800 5400 3000
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 4500 1500 4500 3900
2 1 1 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3375 2700 5775 2625
4 0 0 50 0 0 20 0.0000 4 195 2565 2325 4875 2                  1                  0\001
4 0 0 50 0 0 20 0.0000 4 195 2565 2325 3675 1                  0                  2\001
4 0 0 50 0 0 20 0.0000 4 195 2565 2325 2475 0                  2                  1\001
4 0 0 50 0 0 20 0.0000 4 195 2565 3300 3975 0                  2                  1\001
4 0 0 50 0 0 20 0.0000 4 195 2565 3225 1575 1                  0                  2\001
4 0 0 50 0 0 20 0.0000 4 195 2565 4125 675 2                  1                  0\001
4 0 0 50 0 0 20 0.0000 4 195 2565 4200 1875 0                  2                  1\001
4 0 0 50 0 0 20 0.0000 4 195 2565 4125 3075 1                  0                  2\001
4 0 0 50 0 0 20 0.0000 4 195 2565 3300 2775 2                  1                  0\001


==> figures/magiccubehilbertbasis <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 3000 2400 212 212 3000 2400 3150 2550
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 2987 600 212 212 2987 600 3137 750
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 4797 628 212 212 4797 628 4947 778
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 6580 614 212 212 6580 614 6730 764
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 6592 2424 212 212 6592 2424 6742 2574
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 6600 4200 212 212 6600 4200 6750 4350
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 4800 4187 212 212 4800 4187 4950 4337
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 2976 4208 212 212 2976 4208 3126 4358
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 4838 2430 212 212 4838 2430 4988 2580
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 4211 4823 212 212 4211 4823 4361 4973
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 3611 5348 212 212 3611 5348 3761 5498
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 5936 4823 212 212 5936 4823 6086 4973
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 5411 5348 212 212 5411 5348 5561 5498
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 1811 5348 212 212 1811 5348 1961 5498
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 2411 4748 212 212 2411 4748 2561 4898
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 1811 3548 212 212 1811 3548 1961 3698
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 2411 2948 212 212 2411 2948 2561 3098
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 5942 1215 212 212 5942 1215 6092 1365
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 4200 1200 212 212 4200 1200 4350 1350
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 5386 3557 212 212 5386 3557 5536 3707
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 5986 2957 212 212 5986 2957 6136 3107
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 3586 3557 212 212 3586 3557 3736 3707
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 4186 2957 212 212 4186 2957 4336 3107
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 5400 1800 212 212 5400 1800 5550 1950
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 3576 1808 212 212 3576 1808 3726 1958
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 2381 1173 212 212 2381 1173 2531 1323
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 1800 1800 212 212 1800 1800 1950 1950
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 8420 3565 212 212 8420 3565 8570 3715
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 8420 1840 212 212 8420 1840 8570 1990
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 10231 1818 212 212 10231 1818 10381 1968
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 12031 1818 212 212 12031 1818 12181 1968
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 10231 3618 212 212 10231 3618 10381 3768
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 12031 3618 212 212 12031 3618 12181 3768
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 12631 4818 212 212 12631 4818 12781 4968
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 8400 5400 212 212 8400 5400 8550 5550
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 10200 5413 212 212 10200 5413 10350 5563
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 12043 5374 212 212 12043 5374 12193 5524
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 9075 1200 212 212 9075 1200 9225 1350
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 9635 580 212 212 9635 580 9785 730
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 11400 600 212 212 11400 600 11550 750
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 10875 1200 212 212 10875 1200 11025 1350
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 12675 1200 212 212 12675 1200 12825 1350
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 12675 3075 212 212 12675 3075 12825 3225
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 13275 2400 212 212 13275 2400 13425 2550
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 10800 4813 212 212 10800 4813 10950 4963
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 13200 600 212 212 13200 600 13350 750
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 9675 2400 212 212 9675 2400 9825 2550
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 9023 4814 212 212 9023 4814 9173 4964
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 9566 4168 212 212 9566 4168 9716 4318
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 9000 3000 212 212 9000 3000 9150 3150
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 10800 3000 212 212 10800 3000 10950 3150
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 11400 2400 212 212 11400 2400 11550 2550
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 13165 4180 212 212 13165 4180 13315 4330
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 5432 11974 212 212 5432 11974 5582 12124
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 3000 10800 212 212 3000 10800 3150 10950
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 4800 10800 212 212 4800 10800 4950 10950
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 6600 10800 212 212 6600 10800 6750 10950
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 5400 10200 212 212 5400 10200 5550 10350
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 6000 9600 212 212 6000 9600 6150 9750
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 6600 9000 212 212 6600 9000 6750 9150
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 6600 7200 212 212 6600 7200 6750 7350
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 6000 7800 212 212 6000 7800 6150 7950
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 5475 8400 212 212 5475 8400 5625 8550
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 4800 7200 212 212 4800 7200 4950 7350
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 3000 7200 212 212 3000 7200 3150 7350
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 2400 7800 212 212 2400 7800 2550 7950
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 1800 8400 212 212 1800 8400 1950 8550
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 1800 10200 212 212 1800 10200 1950 10350
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 4275 11325 212 212 4275 11325 4425 11475
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 6075 11400 212 212 6075 11400 6225 11550
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 3632 11974 212 212 3632 11974 3782 12124
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 1800 12000 212 212 1800 12000 1950 12150
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 2400 11400 212 212 2400 11400 2550 11550
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 2475 9600 212 212 2475 9600 2625 9750
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 3000 9000 212 212 3000 9000 3150 9150
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 3675 8400 212 212 3675 8400 3825 8550
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 4200 7800 212 212 4200 7800 4350 7950
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 4800 9000 212 212 4800 9000 4950 9150
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 4200 9600 212 212 4200 9600 4350 9750
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 3600 10200 212 212 3600 10200 3750 10350
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 8424 11992 212 212 8424 11992 8574 12142
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 10224 11992 212 212 10224 11992 10374 12142
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 12024 11992 212 212 12024 11992 12174 12142
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 9024 11392 212 212 9024 11392 9174 11542
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 10824 11392 212 212 10824 11392 10974 11542
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 12549 11392 212 212 12549 11392 12699 11542
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 11400 10800 212 212 11400 10800 11550 10950
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 9600 10800 212 212 9600 10800 9750 10950
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 8400 10200 212 212 8400 10200 8550 10350
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 10200 10200 212 212 10200 10200 10350 10350
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 12000 10200 212 212 12000 10200 12150 10350
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 9000 9600 212 212 9000 9600 9150 9750
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 10800 9600 212 212 10800 9600 10950 9750
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 12600 9600 212 212 12600 9600 12750 9750
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 11400 9000 212 212 11400 9000 11550 9150
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 9600 9000 212 212 9600 9000 9750 9150
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 8400 8400 212 212 8400 8400 8550 8550
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 10200 8400 212 212 10200 8400 10350 8550
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 12000 8400 212 212 12000 8400 12150 8550
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 12600 7800 212 212 12600 7800 12750 7950
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 10800 7800 212 212 10800 7800 10950 7950
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 9000 7800 212 212 9000 7800 9150 7950
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 9600 7200 212 212 9600 7200 9750 7350
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 11400 7200 212 212 11400 7200 11550 7350
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 13200 7200 212 212 13200 7200 13350 7350
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 13210 10823 212 212 13210 10823 13360 10973
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 13135 9023 212 212 13135 9023 13285 9173
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 11392 4224 212 212 11392 4224 11542 4374
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1800 3300 1800 2025
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2025 1800 3375 1800
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3825 1800 5175 1800
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 3375 5400 2025
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 3825 5400 5250
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 3825 5400 5175 5400 5250 5400
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2025 5400 3450 5400
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1800 5175 1800 3825
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2025 3600 3375 3600
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3825 3600 5175 3600
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 2025 3600 3300
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 5100 3600 3825
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 4500 2400 3225
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2625 4800 3975 4800
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4425 4800 5700 4800
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2625 3000 3975 3000
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4425 3000 5850 3000
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2625 1200 3975 1200
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4425 1200 5775 1200
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 2700 2400 1425
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 2775 6000 1425
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 4650 6000 3150
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4200 2775 4200 1425
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4200 4575 4200 3225
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 3975 3000 2625
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 2175 3000 825
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3225 600 4575 600
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5025 600 6375 600
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6600 2175 6600 825
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6600 3975 6600 2625
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5025 4200 6375 4200
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3225 4200 4575 4200
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3225 2400 4650 2400
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5025 2400 6300 2400
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 3900 4800 2700
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 2250 4800 825
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3750 5175 4050 4875
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4350 4650 4725 4275
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5625 5250 5850 4950
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6150 4650 6450 4275
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2025 5250 2325 4950
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2625 4650 2925 4350
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3675 1650 4050 1275
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4275 975 4650 675
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1950 1575 2250 1275
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2550 975 2850 675
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5550 1575 5775 1350
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6075 1050 6450 675
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5550 3450 5850 3150
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6225 2925 6525 2625
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1950 3375 2250 3075
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2625 2775 2850 2550
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12276 5307 12501 5007
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 10425 5400 11775 5400 11850 5400
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8625 5400 10050 5400
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10425 3600 11775 3600
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8625 3600 9975 3600
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10425 1800 11775 1800
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8625 1800 9975 1800
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8400 3375 8400 2025
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8400 3750 8400 5175
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12000 3750 12000 5175
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12000 2025 12000 3450
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10200 2025 10200 3450
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10200 3825 10200 5250
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12825 4650 13125 4275
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2025 12000 3450 12000
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 3825 12000 5175 12000 5250 12000
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5676 11907 5901 11607
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6600 10575 6600 9225
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6600 8700 6600 7350
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 3900 8400 5250 8400 5325 8400
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 2025 8400 3375 8400 3450 8400
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1800 9900 1800 8550
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1800 11700 1800 10350
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 8550 3600 9975
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 8550 5400 9975
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 10350 5400 11775
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 10350 3600 11775
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 2025 10200 3375 10200 3450 10200
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 3825 10200 5175 10200 5250 10200
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 2700 9600 4050 9600 4125 9600
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 4425 9600 5775 9600 5850 9600
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 2625 7800 3975 7800 4050 7800
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 4350 7800 5700 7800 5775 7800
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 5025 7200 6375 7200 6450 7200
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 3225 7200 4575 7200 4650 7200
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6234 11257 6534 10882
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5559 10132 5859 9757
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8550 5250 8850 4950
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9187 4612 9487 4312
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11625 4200 12975 4200
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9750 4200 11100 4200
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12225 3450 12525 3150
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12825 2925 13125 2625
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8587 3412 8887 3112
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9225 2850 9525 2550
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8550 1575 8850 1275
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9150 975 9450 675
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9825 600 11175 600
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11625 600 12975 600
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9300 1200 10650 1200
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11100 1200 12450 1200
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10387 1612 10687 1312
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11062 1012 11362 712
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12262 1612 12562 1312
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12862 1087 13162 787
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 13200 2175 13200 825
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 13200 3900 13200 2550
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12600 2775 12600 1425
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12600 4650 12600 3300
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9600 2175 9600 825
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9600 3900 9600 2550
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 2775 9000 1425
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 4575 9000 3225
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9225 4800 10575 4800
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11025 4800 12375 4800
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9900 2400 11250 2400
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11625 2400 12975 2400
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11400 2175 11400 825
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11400 4050 11400 2700
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10800 2775 10800 1425
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10800 4575 10800 3225
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9225 3000 10575 3000
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11025 3000 12375 3000
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10387 5287 10762 4912
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10987 4687 11362 4312
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 8700 3000 7350
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 10650 3000 9300
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 3225 10800 4575 10800 4650 10800
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 5025 10800 6375 10800 6450 10800
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 9375 2400 8025
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2400 11175 2400 9825
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 2625 11400 3975 11400 4050 11400
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 4500 11400 5850 11400 5925 11400
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 9375 6000 8025
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 11250 6000 9900
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8400 9975 8400 8625
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8400 11775 8400 10425
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 9825 7200 11175 7200 11250 7200
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 11625 7200 12975 7200 13050 7200
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 9225 7800 10575 7800 10650 7800
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 11025 7800 12375 7800 12450 7800
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 8625 8400 9975 8400 10050 8400
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 10425 8400 11775 8400 11850 8400
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 9825 9000 11175 9000 11250 9000
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 9225 9600 10575 9600 10650 9600
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 8625 10200 9975 10200 10050 10200
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 9825 10800 11175 10800 11250 10800
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 10425 10200 11775 10200 11850 10200
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 11625 10800 12975 10800 13050 10800
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 9225 11400 10575 11400 10650 11400
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 11025 11400 12375 11400 12450 11400
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 11025 11400 12375 11400 12450 11400
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 8625 12000 9975 12000 10050 12000
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 10425 12000 11775 12000 11850 12000
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 9375 9000 8025
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9600 8775 9600 7425
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 11175 9000 9825
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9600 10575 9600 9225
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10200 11775 10200 10425
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10200 9975 10200 8625
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10800 9375 10800 8025
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10800 11175 10800 9825
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11400 10575 11400 9225
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11400 8775 11400 7425
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12000 9975 12000 8625
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12600 9375 12600 8025
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12600 11175 12600 9825
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 13200 8700 13200 7350
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 13200 10650 13200 9300
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12801 11232 13026 10932
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12201 11907 12426 11607
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10401 11832 10626 11532
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11001 11232 11226 10932
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9201 11232 9426 10932
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8601 11832 8826 11532
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8601 10032 8826 9732
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9126 9432 9351 9132
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8475 8175 8775 7875
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9075 7575 9375 7275
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1875 8175 2175 7875
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2550 7575 2850 7275
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 3225 9000 4575 9000 4650 9000
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 3825 10200 5175 10200 5250 10200
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 2025 10200 3375 10200 3450 10200
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 5025 9000 6375 9000 6450 9000
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4200 9375 4200 8025
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4200 11175 4200 9825
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 10500 4800 9150
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 8625 4800 7275
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2574 9393 2799 9093
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2250 9750 1950 10125
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6150 9450 6450 9150
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2277 11497 1977 11872
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2562 11184 2787 10884
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5587 8212 5887 7912
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6187 7687 6487 7387
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4425 11175 4650 10875
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3825 11850 4125 11475
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4350 7650 4650 7350
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3750 8175 4050 7875
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10387 8212 10687 7912
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10987 7687 11287 7387
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12187 8212 12487 7912
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12787 7687 13087 7387
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12787 9487 13087 9187
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12187 10087 12487 9787
2 1 0 1 9 7 50 0 -1 0.000 0 0 -1 0 0 2
	 12000 11850 12000 10500
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 11025 9600 12375 9600 12450 9600
2 1 0 1 10 7 50 0 -1 0.000 0 0 -1 0 0 3
	 11625 9000 12975 9000 13050 9000
4 0 18 50 0 0 20 0.0000 4 195 135 1725 5475 2\001
4 0 18 50 0 0 20 0.0000 4 195 135 3525 5475 1\001
4 0 18 50 0 0 20 0.0000 4 195 135 5325 5475 0\001
4 0 18 50 0 0 20 0.0000 4 195 135 3525 3675 0\001
4 0 18 50 0 0 20 0.0000 4 195 135 1725 3675 1\001
4 0 18 50 0 0 20 0.0000 4 195 135 5325 3675 2\001
4 0 18 50 0 0 20 0.0000 4 195 135 4125 3075 1\001
4 0 18 50 0 0 20 0.0000 4 195 135 2325 1275 1\001
4 0 18 50 0 0 20 0.0000 4 195 135 2325 4875 0\001
4 0 18 50 0 0 20 0.0000 4 195 135 4125 4875 2\001
4 0 18 50 0 0 20 0.0000 4 195 135 5925 4875 1\001
4 0 18 50 0 0 20 0.0000 4 195 135 5925 3075 0\001
4 0 18 50 0 0 20 0.0000 4 195 135 2325 3075 2\001
4 0 18 50 0 0 20 0.0000 4 195 135 4125 1275 0\001
4 0 18 50 0 0 20 0.0000 4 195 135 5925 1275 2\001
4 0 18 50 0 0 20 0.0000 4 195 135 4725 4275 0\001
4 0 18 50 0 0 20 0.0000 4 195 135 2925 2475 0\001
4 0 18 50 0 0 20 0.0000 4 195 135 6525 675 0\001
4 0 18 50 0 0 20 0.0000 4 195 135 2925 675 2\001
4 0 18 50 0 0 20 0.0000 4 195 135 4725 675 1\001
4 0 18 50 0 0 20 0.0000 4 195 135 6525 2475 1\001
4 0 18 50 0 0 20 0.0000 4 195 135 6525 4275 2\001
4 0 18 50 0 0 20 0.0000 4 195 135 2925 4275 1\001
4 0 18 50 0 0 20 0.0000 4 195 135 4725 2475 2\001
4 0 18 50 0 0 20 0.0000 4 195 135 5325 1875 1\001
4 0 18 50 0 0 20 0.0000 4 195 135 3525 1875 2\001
4 0 18 50 0 0 20 0.0000 4 195 135 1725 1875 0\001
4 0 18 50 0 0 20 0.0000 4 195 135 8325 3675 1\001
4 0 18 50 0 0 20 0.0000 4 195 135 10125 3675 1\001
4 0 18 50 0 0 20 0.0000 4 195 135 11925 3675 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 8325 5475 2\001
4 0 19 50 0 0 20 0.0000 4 195 135 10125 5475 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 11925 5475 0\001
4 0 19 50 0 0 20 0.0000 4 195 135 8325 1950 0\001
4 0 19 50 0 0 20 0.0000 4 195 135 10125 1875 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 12000 1875 2\001
4 0 19 50 0 0 20 0.0000 4 195 135 12600 4875 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 12600 3150 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 9000 1275 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 10800 1275 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 12600 1275 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 11325 4275 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 13125 4275 2\001
4 0 19 50 0 0 20 0.0000 4 195 135 9600 2475 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 13200 2475 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 9600 675 2\001
4 0 19 50 0 0 20 0.0000 4 195 135 11325 675 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 10725 4875 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 13125 675 0\001
4 0 19 50 0 0 20 0.0000 4 195 135 8925 3075 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 10725 3075 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 11325 2475 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 8925 4875 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 9525 4275 0\001
4 0 0 50 0 0 20 0.0000 4 240 315 4650 150 [8]\001
4 0 19 50 0 0 20 0.0000 4 195 135 5400 12075 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 3600 10275 0\001
4 0 19 50 0 0 20 0.0000 4 195 135 5400 10275 2\001
4 0 19 50 0 0 20 0.0000 4 195 135 3600 8475 2\001
4 0 19 50 0 0 20 0.0000 4 195 135 5400 8475 0\001
4 0 19 50 0 0 20 0.0000 4 195 135 1725 8475 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 1725 10275 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 4200 11475 2\001
4 0 19 50 0 0 20 0.0000 4 195 135 6000 11475 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 4125 9675 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 5925 9675 0\001
4 0 19 50 0 0 20 0.0000 4 195 135 2400 9675 2\001
4 0 19 50 0 0 20 0.0000 4 195 135 2325 7875 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 4125 7875 0\001
4 0 19 50 0 0 20 0.0000 4 195 135 5925 7875 2\001
4 0 19 50 0 0 20 0.0000 4 195 135 2925 10875 2\001
4 0 19 50 0 0 20 0.0000 4 195 135 4725 10875 0\001
4 0 19 50 0 0 20 0.0000 4 195 135 6525 10875 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 2925 9075 0\001
4 0 19 50 0 0 20 0.0000 4 195 135 4725 9075 2\001
4 0 19 50 0 0 20 0.0000 4 195 135 6525 9075 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 2925 7275 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 4725 7275 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 6525 7275 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 1725 12075 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 2325 11475 0\001
4 0 19 50 0 0 20 0.0000 4 195 135 3525 12075 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 10125 12075 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 11925 12075 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 8925 11475 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 10725 11475 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 12525 11475 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 8325 10275 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 10125 10275 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 11925 10275 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 8325 12075 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 8325 8475 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 10125 8475 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 11925 8475 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 8925 9675 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 10725 9675 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 12525 9675 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 8925 7875 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 10725 7875 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 12525 7875 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 9525 10875 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 11325 10875 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 9525 9075 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 11325 9075 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 13125 9075 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 9525 7275 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 11325 7275 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 13125 7275 1\001
4 0 19 50 0 0 20 0.0000 4 195 135 13125 10875 1\001
4 0 0 50 0 0 20 0.0000 4 240 315 11325 6675 [1]\001
4 0 0 50 0 0 20 0.0000 4 240 315 3900 6825 [8]\001
4 0 0 50 0 0 20 0.0000 4 240 315 11325 225 [2]\001


==> figures/notpositive <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 3300 2400 75 75 3300 2400 3300 2475
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 2400 3300 75 75 2400 3300 2400 3375
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 4200 3300 75 75 4200 3300 4200 3375
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 2400 4200 3300
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 4
	 3300 2325 3150 2025 3450 2025 3300 2325
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 4
	 2400 3375 2550 3675 2250 3675 2400 3375
	 0.000 -1.000 -1.000 0.000
4 0 0 50 0 0 20 0.0000 4 195 135 3525 2475 1\001
4 0 0 50 0 0 20 0.0000 4 195 135 2100 3375 3\001
4 0 0 50 0 0 20 0.0000 4 195 135 4350 3375 2\001


==> figures/octwithorient <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 2400 2100 75 75 2400 2100 2475 2100
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 1800 2700 75 75 1800 2700 1875 2700
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 3000 2700 75 75 3000 2700 3075 2700
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 4200 1500 75 75 4200 1500 4275 1500
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 600 1500 75 75 600 1500 675 1500
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 2400 4500 75 75 2400 4500 2475 4500
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 7200 1500 75 75 7200 1500 7275 1500
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 7200 2100 75 75 7200 2100 7275 2100
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 7200 3300 75 75 7200 3300 7275 3300
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 7200 3900 75 75 7200 3900 7275 3900
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 7200 4500 75 75 7200 4500 7275 4500
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 7200 2700 75 75 7200 2700 7275 2700
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 8700 1500 75 75 8700 1500 8775 1500
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 8700 2100 75 75 8700 2100 8775 2100
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 8700 2700 75 75 8700 2700 8775 2700
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 8700 3300 75 75 8700 3300 8775 3300
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 8700 3900 75 75 8700 3900 8775 3900
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 8700 4500 75 75 8700 4500 8775 4500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 675 1500 4050 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 4125 1575 2550 4425
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2325 4500 675 1650
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2925 2700 1950 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1875 2625 2325 2175
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2475 2175 2925 2550
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 675 1575 2325 2025
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 1725 2700 750 1650
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2475 2025 3975 1575
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 3900 1650 3150 2550
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 3000 2775 2475 4350
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2397 4426 1797 2851
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 1500 8700 2100
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 1500 8700 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 2100 8700 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 2100 8700 4500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 2700 8700 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 2700 8700 3900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 3300 8625 2100
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 3300 8700 4500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 3900 8700 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 3900 8700 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 4500 8700 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 4500 8700 3900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 1 1 2
	0 0 1.00 60.00 120.00
	0 0 1.00 60.00 120.00
	 4200 3300 5700 3300
4 0 0 50 0 0 15 0.0000 4 150 105 525 1350 1\001
4 0 0 50 0 0 15 0.0000 4 150 105 4200 1350 2\001
4 0 0 50 0 0 15 0.0000 4 150 105 2400 1875 4\001
4 0 0 50 0 0 15 0.0000 4 150 105 2400 4800 3\001
4 0 0 50 0 0 15 0.0000 4 150 105 9000 2175 2\001
4 0 0 50 0 0 15 0.0000 4 150 105 9000 2775 3\001
4 0 0 50 0 0 15 0.0000 4 150 105 9000 3375 4\001
4 0 0 50 0 0 15 0.0000 4 150 105 6825 3975 5\001
4 0 0 50 0 0 15 0.0000 4 150 105 9000 3975 5\001
4 0 0 50 0 0 15 0.0000 4 150 105 6825 4500 6\001
4 0 0 50 0 0 15 0.0000 4 150 105 9000 4500 6\001
4 0 0 50 0 0 15 0.0000 4 150 105 1500 2775 5\001
4 0 0 50 0 0 15 0.0000 4 150 105 3225 2775 6\001
4 0 0 50 0 0 15 0.0000 4 150 105 9000 1575 1\001
4 0 0 50 0 0 15 0.0000 4 150 105 6825 2775 3\001
4 0 0 50 0 0 15 0.0000 4 150 105 6825 3375 4\001
4 0 0 50 0 0 15 0.0000 4 150 105 6825 1575 1\001
4 0 0 50 0 0 15 0.0000 4 150 105 6900 2175 2\001


==> figures/oddmagicconstruct <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 5
	 1800 3300 1800 4800 3300 4800 3300 3300 1800 3300
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 2100 3300 2100 4800
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 2400 4800 2400 3300
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 2700 3300 2700 4800
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3000 3300 3000 4800
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1800 3600 3300 3600
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1800 3900 3300 3900
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1800 4200 3300 4200
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1800 4500 3300 4500
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5400 3300 5400 4800
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5700 3300 5700 4800
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 6000 3300 6000 4800
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 6300 3300 6300 4800
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5100 3600 6600 3600
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5100 3900 6600 3900
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5100 4200 6600 4200
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5100 4500 6600 4500
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 5
	 8400 3300 8400 4800 9900 4800 9900 3300 8400 3300
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8400 3900 9900 3900
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8400 3600 9900 3600
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8400 4200 9900 4200
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8400 4500 9900 4500
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9600 3300 9600 4800
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9300 3300 9300 4800
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 9000 3300 9000 4800
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 8700 3300 8700 4800
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 1200 3900 1200 4200 1500 4200 1500 3900 1200 3900
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 1500 3600 1500 3900 1800 3900 1800 3600 1500 3600
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 2100 3000 2100 3300 2400 3300 2400 3000 2100 3000
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 2400 2700 2400 3000 2700 3000 2700 2700 2400 2700
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 2700 3000 2700 3300 3000 3300 3000 3000 2700 3000
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 3300 3600 3300 3900 3600 3900 3600 3600 3300 3600
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 3600 3900 3600 4200 3900 4200 3900 3900 3600 3900
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 3300 4200 3300 4500 3600 4500 3600 4200 3300 4200
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 2700 4800 2700 5100 3000 5100 3000 4800 2700 4800
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 2400 5100 2400 5400 2700 5400 2700 5100 2400 5100
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 2100 4800 2100 5100 2400 5100 2400 4800 2100 4800
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 1500 4200 1500 4500 1800 4500 1800 4200 1500 4200
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 4800 3600 4800 3900 5100 3900 5100 3600 4800 3600
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 4500 3900 4500 4200 4800 4200 4800 3900 4500 3900
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 4800 4200 4800 4500 5100 4500 5100 4200 4800 4200
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 6600 3600 6600 3900 6900 3900 6900 3600 6600 3600
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 6900 3900 6900 4200 7200 4200 7200 3900 6900 3900
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 6600 4200 6600 4500 6900 4500 6900 4200 6600 4200
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2550 5025 2550 3675
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2850 4800 2850 3375
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 2175 4800 2175 3450
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 5
	 5100 3300 5100 4800 6600 4800 6600 3300 5100 3300
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 5400 3000 5400 3300 5700 3300 5700 3000 5400 3000
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 6000 3000 6000 3300 6300 3300 6300 3000 6000 3000
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 5700 2700 5700 3000 6000 3000 6000 2700 5700 2700
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 5550 3225 5550 4650
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 6225 3225 6225 4650
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 5850 3000 5850 4425
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 8100 3600 8100 3900 8400 3900 8400 3600 8100 3600
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 8100 4200 8100 4500 8400 4500 8400 4200 8100 4200
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 7800 3900 7800 4200 8100 4200 8100 3900 7800 3900
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 9900 3600 9900 3900 10200 3900 10200 3600 9900 3600
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 9900 4200 9900 4500 10200 4500 10200 4200 9900 4200
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 10200 3900 10200 4200 10500 4200 10500 3900 10200 3900
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 8400 3750 9825 3750
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 8100 4050 9450 4050
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 8400 4350 9825 4350
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1800 6300 3300 6300
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1800 6600 3300 6600
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1800 6900 3300 6900
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5100 6300 6600 6300
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5100 6600 6600 6600
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5100 6900 6600 6900
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 5
	 1800 6300 1800 7800 3300 7800 3300 6300 1800 6300
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 2100 6300 2100 7800
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 2400 6300 2400 7800
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 2700 6300 2700 7800
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 3000 6300 3000 7800
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 3300 7350 1875 7350
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 3300 7200 3300 7500 3600 7500 3600 7200 3300 7200
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 3600 6900 3600 7200 3900 7200 3900 6900 3600 6900
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 3300 6600 3300 6900 3600 6900 3600 6600 3300 6600
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1800 7200 3300 7200
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 3300 6750 1875 6750
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 1 0 2
	0 0 1.00 60.00 120.00
	 3600 7050 2175 7050
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 1800 7500 3300 7500
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 5
	 5100 6300 5100 7800 6600 7800 6600 6300 5100 6300
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5400 6300 5400 7800
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5700 6300 5700 7800
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 6000 6300 6000 7800
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 6300 6300 6300 7800
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5100 7200 6600 7200
2 1 0 1 0 7 50 0 -1 4.000 0 0 -1 0 0 2
	 5100 7500 6600 7500
4 0 0 50 0 0 12 0.0000 4 135 90 1350 4125 1\001
4 0 0 50 0 0 12 0.0000 4 135 90 1650 3825 2\001
4 0 0 50 0 0 12 0.0000 4 135 90 1950 3525 3\001
4 0 0 50 0 0 12 0.0000 4 135 90 2550 2925 5\001
4 0 0 50 0 0 12 0.0000 4 135 90 1650 4425 6\001
4 0 0 50 0 0 12 0.0000 4 135 90 1950 4125 7\001
4 0 0 50 0 0 12 0.0000 4 135 90 2250 3825 8\001
4 0 0 50 0 0 12 0.0000 4 135 180 2475 4125 13\001
4 0 0 50 0 0 12 0.0000 4 135 180 2775 3825 14\001
4 0 0 50 0 0 12 0.0000 4 135 180 3075 3525 15\001
4 0 0 50 0 0 12 0.0000 4 135 180 2175 5025 16\001
4 0 0 50 0 0 12 0.0000 4 135 180 2475 4725 17\001
4 0 0 50 0 0 12 0.0000 4 135 180 2775 4425 18\001
4 0 0 50 0 0 12 0.0000 4 135 180 3075 4125 19\001
4 0 0 50 0 0 12 0.0000 4 135 180 3675 4125 25\001
4 0 0 50 0 0 12 0.0000 4 135 90 2175 3225 4\001
4 0 0 50 0 0 12 0.0000 4 135 180 2775 3225 10\001
4 0 0 50 0 0 12 0.0000 4 135 90 2475 3525 9\001
4 0 0 50 0 0 12 0.0000 4 135 180 1875 4725 11\001
4 0 0 50 0 0 12 0.0000 4 135 180 2175 4425 12\001
4 0 0 50 0 0 12 0.0000 4 135 180 3375 3825 20\001
4 0 0 50 0 0 12 0.0000 4 135 180 2475 5325 21\001
4 0 0 50 0 0 12 0.0000 4 135 180 2775 5025 22\001
4 0 0 50 0 0 12 0.0000 4 135 180 3075 4725 23\001
4 0 0 50 0 0 12 0.0000 4 135 180 3375 4425 24\001
4 0 0 50 0 0 12 0.0000 4 135 1395 5175 3525 3     16   9    22   15\001
4 0 0 50 0 0 12 0.0000 4 135 810 5475 3825  8    21   14\001
4 0 0 50 0 0 12 0.0000 4 135 90 4950 3825 2\001
4 0 0 50 0 0 12 0.0000 4 135 90 4650 4125 1\001
4 0 0 50 0 0 12 0.0000 4 135 90 4950 4425 6\001
4 0 0 50 0 0 12 0.0000 4 135 180 6675 3825 20\001
4 0 0 50 0 0 12 0.0000 4 135 180 6975 4125 25\001
4 0 0 50 0 0 12 0.0000 4 135 180 6675 4425 24\001
4 0 0 50 0 0 12 0.0000 4 135 1350 5175 4125 7           13         19\001
4 0 0 50 0 0 12 0.0000 4 135 1395 8475 3525 3     16   9    22   15\001
4 0 0 50 0 0 12 0.0000 4 135 1350 8475 4725 11   4    17   10  23\001
4 0 0 50 0 0 12 0.0000 4 135 90 5550 3225 4\001
4 0 0 50 0 0 12 0.0000 4 135 180 6075 3225 10\001
4 0 0 50 0 0 12 0.0000 4 135 90 5775 2925 5\001
4 0 0 50 0 0 12 0.0000 4 135 180 5475 4425 12\001
4 0 0 50 0 0 12 0.0000 4 135 180 6075 4425 18\001
4 0 0 50 0 0 12 0.0000 4 135 180 5175 4725 11\001
4 0 0 50 0 0 12 0.0000 4 135 180 5775 4725 17\001
4 0 0 50 0 0 12 0.0000 4 135 180 6375 4725 23\001
4 0 0 50 0 0 12 0.0000 4 135 810 8775 3825  8    21   14\001
4 0 0 50 0 0 12 0.0000 4 135 1350 8475 4125 7           13         19\001
4 0 0 50 0 0 12 0.0000 4 135 810 8775 4425 12    5    18\001
4 0 0 50 0 0 12 0.0000 4 135 90 8250 3825 2\001
4 0 0 50 0 0 12 0.0000 4 135 90 7950 4125 1\001
4 0 0 50 0 0 12 0.0000 4 135 90 8250 4425 6\001
4 0 0 50 0 0 12 0.0000 4 135 180 9975 3825 20\001
4 0 0 50 0 0 12 0.0000 4 135 180 10275 4125 25\001
4 0 0 50 0 0 12 0.0000 4 135 180 9975 4425 24\001
4 0 0 50 0 0 12 0.0000 4 135 1350 1875 7725 11   4    17   10  23\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2175 7425 12    5    18   6\001
4 0 0 50 0 0 12 0.0000 4 135 180 3375 7425 24\001
4 0 0 50 0 0 12 0.0000 4 135 180 3675 7125 25\001
4 0 0 50 0 0 12 0.0000 4 135 1395 1875 7125 7            13    1   19\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2175 6825  8    21   14   2\001
4 0 0 50 0 0 12 0.0000 4 135 180 3375 6825 20\001
4 0 0 50 0 0 12 0.0000 4 135 1395 1875 6525 3     16   9    22   15\001
4 0 0 50 0 0 12 0.0000 4 135 1350 5175 7725 11   4    17   10  23\001
4 0 0 50 0 0 12 0.0000 4 135 1350 5175 7425 24  12    5    18    6\001
4 0 0 50 0 0 12 0.0000 4 135 1395 5175 7125 7    25    13   1    19\001
4 0 0 50 0 0 12 0.0000 4 135 1305 5175 6825 20    8    21  14   2\001
4 0 0 50 0 0 12 0.0000 4 135 1395 5175 6525 3     16   9    22   15\001
4 0 0 50 0 0 20 0.0000 4 255 690 2250 2475 Step 1\001
4 0 0 50 0 0 20 0.0000 4 255 690 5550 2475 Step 2\001
4 0 0 50 0 0 20 0.0000 4 255 750 8925 2475 Step  3\001
4 0 0 50 0 0 20 0.0000 4 255 750 2250 6075 Step  4\001
4 0 0 50 0 0 20 0.0000 4 255 750 5550 6075 Step  5\001


==> figures/panjainaconstruct <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 900 2700 900 3900 2100 3900 2100 2700 900 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 3000 2700 3000 3900 4200 3900 4200 2700 3000 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 5100 2700 5100 3900 6300 3900 6300 2700 5100 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 7200 2700 7200 3900 8400 3900 8400 2700 7200 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 3000 8400 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 3300 8400 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 3600 8400 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 3000 6300 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 3300 6300 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 3600 6300 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 3000 4200 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 3300 4200 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 3600 4200 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 3000 2100 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 3300 2100 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 3600 2100 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 3900 1200 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1800 3900 1800 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 3900 3300 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 3900 3600 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3900 3900 3900 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 3900 5400 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5700 3900 5700 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 3900 6000 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7500 3900 7500 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 3900 7800 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8100 3900 8100 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 -1200 2700 -1200 3900 0 3900 0 2700 -1200 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 -3300 2700 -3300 3900 -2100 3900 -2100 2700 -3300 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -3000 3900 -3000 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -2700 3900 -2700 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -2400 3900 -2400 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -900 3900 -900 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -3300 3000 -2100 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -3300 3300 -2100 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -3300 3600 -2100 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1200 3000 0 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1200 3300 0 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -1200 3600 0 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -600 3900 -600 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -300 3900 -300 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1500 3900 1500 2700
4 0 0 50 0 0 12 0.0000 4 135 1125 7275 2925 7    12     1   14 \001
4 0 0 50 0 0 12 0.0000 4 135 1080 7275 3225 2    13    8    11\001
4 0 0 50 0 0 12 0.0000 4 135 1035 7275 3525 16   3    10    5\001
4 0 0 50 0 0 12 0.0000 4 135 1035 7275 3825  9     6   15    4\001
4 0 0 50 0 0 18 0.0000 4 45 150 6675 3375 =\001
4 0 0 50 0 0 20 0.0000 4 195 285 300 3375 +2\001
4 0 0 50 0 0 20 0.0000 4 195 285 -1875 3375 +8\001
4 0 0 50 0 0 20 0.0000 4 135 150 2400 3375 +\001
4 0 0 50 0 0 20 0.0000 4 195 285 4500 3375 +5\001
4 0 0 50 0 0 12 0.0000 4 135 990 -3225 2925 0      1    0    1\001
4 0 0 50 0 0 12 0.0000 4 135 990 -3225 3225 1      0    1    0\001
4 0 0 50 0 0 12 0.0000 4 135 990 -3225 3525 1      0    1    0\001
4 0 0 50 0 0 12 0.0000 4 135 990 -3225 3825 0      1    0    1\001
4 0 0 50 0 0 12 0.0000 4 135 990 -1125 2925 0      1    0    1\001
4 0 0 50 0 0 12 0.0000 4 135 990 -1125 3225 0      1    0    1\001
4 0 0 50 0 0 12 0.0000 4 135 990 -1125 3525 1      0    1    0\001
4 0 0 50 0 0 12 0.0000 4 135 990 -1125 3825 1      0    1    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 975 2925  1    1     0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1170 975 3225 0     0     1     1   \001
4 0 0 50 0 0 12 0.0000 4 135 1035 975 3525  1    1     0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1170 975 3825 0     0     1     1   \001
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 2925  0    1     1     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 3225 1      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 3525  0    1     1     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 3075 3825 1      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 5175 2925 1      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 5175 3525 1      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 5175 3225  0    1     1     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 5175 3825  0    1     1     0\001


==> figures/panmagic4hilb <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 900 600 900 1800 2100 1800 2100 600 900 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 1
	 1200 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 600 1200 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 900 2100 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 1200 2100 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 1500 2100 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1500 600 1500 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1800 600 1800 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 2700 600 2700 1800 3900 1800 3900 600 2700 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 4500 600 4500 1800 5700 1800 5700 600 4500 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 6300 600 6300 1800 7500 1800 7500 600 6300 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 900 2400 900 3600 2100 3600 2100 2400 900 2400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 2700 2400 2700 3600 3900 3600 3900 2400 2700 2400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 4500 2400 4500 3600 5700 3600 5700 2400 4500 2400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 6300 2400 6300 3600 7500 3600 7500 2400 6300 2400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 600 3000 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 600 3300 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 600 3600 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 600 4800 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 600 5100 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 600 5400 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6600 600 6600 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 600 6900 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 600 7200 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 2400 1200 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1500 2400 1500 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1800 2400 1800 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 2400 3000 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 2400 3300 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 2400 3600 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 2400 4800 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 2400 5100 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 2400 5400 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6600 2400 6600 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 2400 6900 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 2400 7200 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 900 3900 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 1200 3900 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 1500 3900 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4500 900 5700 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4500 1200 5700 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4500 1500 5700 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6300 900 7500 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6300 1200 7500 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6300 1500 7500 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 2700 2100 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 3000 2100 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 3300 2100 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 2700 3900 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 3000 3900 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 3300 3900 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4500 2700 5700 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4500 3000 5700 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4500 3300 5700 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6300 2700 7500 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6300 3000 7500 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6300 3300 7500 3300
4 0 0 50 0 0 12 0.0000 4 135 1035 975 825 1      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1080 975 1125 0      1    1     0 \001
4 0 0 50 0 0 12 0.0000 4 135 1035 975 1425 1      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1080 975 1725 0      1    1     0 \001
4 0 0 50 0 0 12 0.0000 4 135 1035 4575 825  0    0     1     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 4575 1125 1      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 4575 1425  0    0     1     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 4575 1725 1      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 990 975 3225  1     0    1    0\001
4 0 0 50 0 0 12 0.0000 4 135 990 975 3525  1     0    1    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 975 2625  0     1    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 975 2925  0     1    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 990 2775 2625  1     0    1    0\001
4 0 0 50 0 0 12 0.0000 4 135 990 2775 2925  1     0    1    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2775 3225  0     1    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2775 3525  0     1    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 990 4575 2625  1     0    1    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 4575 2925  0     1    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 4575 3225  0     1    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 990 4575 3525  1     0    1    0\001
4 0 0 50 0 0 12 0.0000 4 135 1080 2775 825 0      1    1     0 \001
4 0 0 50 0 0 12 0.0000 4 135 1080 2775 1425 0      1    1     0 \001
4 0 0 50 0 0 12 0.0000 4 135 1035 2775 1125 1      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 2775 1725 1      0    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 6375 2625  0     1    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 6375 3525  0     1    0     1\001
4 0 0 50 0 0 12 0.0000 4 135 990 6375 2925  1     0    1    0\001
4 0 0 50 0 0 12 0.0000 4 135 990 6375 3225  1     0    1    0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 6375 825 1      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 6375 1425 1      1    0     0\001
4 0 0 50 0 0 12 0.0000 4 135 1035 6375 1125  0    0     1     1\001
4 0 0 50 0 0 12 0.0000 4 135 1035 6375 1725  0    0     1     1\001


==> figures/panmagic5hilb <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 600 600 600 2100 2100 2100 2100 600 600 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 2100 900 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 900 2100 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 2700 600 2700 2100 4200 2100 4200 600 2700 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 4800 600 4800 2100 6300 2100 6300 600 4800 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 6900 600 6900 2100 8400 2100 8400 600 6900 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 9000 600 9000 2100 10500 2100 10500 600 9000 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 600 2700 600 4200 2100 4200 2100 2700 600 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 2700 2700 2700 4200 4200 4200 4200 2700 2700 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 4800 2700 4800 4200 6300 4200 6300 2700 4800 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 6900 2700 6900 4200 8400 4200 8400 2700 6900 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 5
	 9000 2700 9000 4200 10500 4200 10500 2700 9000 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 1200 2100 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 1500 2100 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 1800 2100 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 2100 1200 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1500 2100 1500 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1800 2100 1800 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 2100 3000 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 2100 3300 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 2100 3600 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3900 2100 3900 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 2100 5100 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 2100 5400 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5700 2100 5700 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 2100 6000 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7500 2100 7500 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 2100 7800 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8100 2100 8100 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 2100 7200 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9300 2100 9300 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9600 2100 9600 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9900 2100 9900 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10200 2100 10200 600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 900 4200 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 1200 4200 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 1500 4200 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 1800 4200 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 900 6300 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 1200 6300 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 1500 6300 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 1800 6300 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 3000 2100 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 3300 2100 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 3600 2100 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 600 3900 2100 3900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 3000 4200 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 3300 4200 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 3600 4200 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 3900 4200 3900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 3000 6300 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 3300 6300 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 3600 6300 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 3900 6300 3900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 3000 8400 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 3300 8400 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 3600 8400 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 3900 8400 3900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 3000 10500 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 3300 10500 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 3600 10500 3600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 3900 10500 3900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 900 8400 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 1200 8400 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 1500 8400 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6900 1800 8400 1800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 900 4200 900 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 4200 1200 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1500 4200 1500 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1800 4200 1800 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3000 4200 3000 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 4200 3300 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3600 4200 3600 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3900 4200 3900 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5100 4200 5100 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 4200 5400 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5700 4200 5700 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6000 4200 6000 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7200 4200 7200 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7500 4200 7500 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7800 4200 7800 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 8100 4200 8100 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9300 4200 9300 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9600 4200 9600 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9900 4200 9900 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 10200 4200 10200 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 900 10500 900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 1200 10500 1200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 1500 10500 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 9000 1800 10500 1800
4 0 0 50 0 0 12 0.0000 4 135 1305 675 825  1    0     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1305 675 1125  0     0    1     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1530 675 1425  0     0    0     0     1    \001
4 0 0 50 0 0 12 0.0000 4 135 1305 675 1725  0    1     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1395 675 2025  0     0    0     1    0  \001
4 0 0 50 0 0 12 0.0000 4 135 1305 2775 825  1    0     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1395 2775 1125  0     0    0     1    0  \001
4 0 0 50 0 0 12 0.0000 4 135 1305 2775 1425  0    1     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1530 2775 1725  0     0    0     0     1    \001
4 0 0 50 0 0 12 0.0000 4 135 1305 2775 2025  0     0    1     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1305 4875 825  0    1     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1395 4875 1125  0     0    0     1    0  \001
4 0 0 50 0 0 12 0.0000 4 135 1305 4875 1425  1    0     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1305 4875 1725  0     0    1     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1530 4875 2025  0     0    0     0     1    \001
4 0 0 50 0 0 12 0.0000 4 135 1305 6975 825  0    1     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1530 6975 1125  0     0    0     0     1    \001
4 0 0 50 0 0 12 0.0000 4 135 1305 6975 1425  0     0    1     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1305 6975 1725  1    0     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1395 6975 2025  0     0    0     1    0  \001
4 0 0 50 0 0 12 0.0000 4 135 1305 9075 825  0     0    1     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1305 9075 1125  1    0     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1395 9075 1425  0     0    0     1    0  \001
4 0 0 50 0 0 12 0.0000 4 135 1305 9075 1725  0    1     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1530 9075 2025  0     0    0     0     1    \001
4 0 0 50 0 0 12 0.0000 4 135 1305 675 2925  0     0    1     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1530 675 3225  0     0    0     0     1    \001
4 0 0 50 0 0 12 0.0000 4 135 1305 675 3525  0    1     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1395 675 3825  0     0    0     1    0  \001
4 0 0 50 0 0 12 0.0000 4 135 1305 675 4125  1    0     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1395 2775 2925  0     0    0     1    0  \001
4 0 0 50 0 0 12 0.0000 4 135 1305 2775 3225  1    0     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1305 2775 3525  0     0    1     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1530 2775 3825  0     0    0     0     1    \001
4 0 0 50 0 0 12 0.0000 4 135 1305 2775 4125  0    1     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1395 4875 2925  0     0    0     1    0  \001
4 0 0 50 0 0 12 0.0000 4 135 1305 4875 3225  0    1     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1530 4875 3525  0     0    0     0     1    \001
4 0 0 50 0 0 12 0.0000 4 135 1305 4875 3825  0     0    1     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1305 4875 4125  1    0     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1530 6975 2925  0     0    0     0     1    \001
4 0 0 50 0 0 12 0.0000 4 135 1530 9075 2925  0     0    0     0     1    \001
4 0 0 50 0 0 12 0.0000 4 135 1305 6975 3225  0    1     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1305 9075 4125  0    1     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1395 6975 3525  0     0    0     1    0  \001
4 0 0 50 0 0 12 0.0000 4 135 1395 9075 3825  0     0    0     1    0  \001
4 0 0 50 0 0 12 0.0000 4 135 1305 6975 3825  1    0     0     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1305 6975 4125  0     0    1     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1305 9075 3225  0     0    1     0    0\001
4 0 0 50 0 0 12 0.0000 4 135 1305 9075 3525  1    0     0     0    0\001


==> figures/pansymm3hilbertbasis <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 2700 2700 75 75 2700 2700 2700 2775
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 1800 2700 75 75 1800 2700 1800 2775
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 2250 3600 75 75 2250 3600 2250 3675
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 1800 2700 2700 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2250 3600 1800 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2250 3600 2700 2700
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 3675 3150 4275 3150
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 3375 2400 3375 3600 5250 3600 5250 2400 3375 2400
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 4
	 2250 3600 2400 3900 2100 3900 2250 3600
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 4
	 2730 2685 2580 2385 2880 2385 2730 2685
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 4
	 1770 2640 1620 2340 1920 2340 1770 2640
	 0.000 -1.000 -1.000 0.000
4 0 0 50 0 0 12 0.0000 4 135 90 1575 2775 2\001
4 0 0 50 0 0 12 0.0000 4 135 90 2925 2775 3\001
4 0 0 50 0 0 12 0.0000 4 135 90 1950 3675 1\001
4 0 0 50 0 0 12 0.0000 4 180 390 3750 2925 Edge\001
4 0 0 50 0 0 12 0.0000 4 135 420 4575 2925 Label\001
4 0 0 50 0 0 12 0.0000 4 135 90 4725 3225 1\001
4 0 0 50 0 0 15 0.0000 4 195 255 2100 2325 [1]\001


==> figures/pansymm4hilbertbasis <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 1200 1500 75 75 1200 1500 1200 1575
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 1200 2400 75 75 1200 2400 1200 2475
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 2100 2400 75 75 2100 2400 2100 2475
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 2100 1500 75 75 2100 1500 2100 1575
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 3300 2400 75 75 3300 2400 3300 2475
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 3300 1500 75 75 3300 1500 3300 1575
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 4200 1500 75 75 4200 1500 4200 1575
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 4200 2400 75 75 4200 2400 4200 2475
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 1500 2100 2400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 2400 2100 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 3
	 1200 1500 1200 2400 1125 2400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 2400 2100 2400
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2100 2400 2100 1500
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 1500 2100 1500
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 6300 1350 5700 1350
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 6300 1650 5700 1650
2 1 0 3 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5700 1950 6300 1950
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 5550 600 5550 2400 7350 2400 7350 600 5550 600
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 3300 1575 3300 2400
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 4200 1500 3300 2400
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 4200 2400 4200 1500
2 1 0 3 0 7 50 0 -1 6.000 0 0 -1 0 0 2
	 3300 2400 4200 2400
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 3300 1500 4200 2400
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 3300 1500 4200 1500
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 4
	 1200 1425 1050 1125 1350 1125 1200 1425
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 4
	 2100 1425 1950 1125 2250 1125 2100 1425
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 4
	 1200 2400 1350 2700 1050 2700 1200 2400
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 4
	 2100 2400 2250 2700 1950 2700 2100 2400
	 0.000 -1.000 -1.000 0.000
3 2 0 3 0 7 50 0 -1 0.000 0 0 0 4
	 3330 1485 3180 1185 3480 1185 3330 1485
	 0.000 -1.000 -1.000 0.000
3 2 0 3 0 7 50 0 -1 0.000 0 0 0 4
	 4200 1500 4050 1200 4350 1200 4200 1500
	 0.000 -1.000 -1.000 0.000
3 2 2 1 0 7 50 0 -1 3.000 0 0 0 4
	 3300 2475 3450 2775 3150 2775 3300 2475
	 0.000 -1.000 -1.000 0.000
3 2 2 1 0 7 50 0 -1 3.000 0 0 0 4
	 4200 2475 4350 2775 4050 2775 4200 2475
	 0.000 -1.000 -1.000 0.000
4 0 0 50 0 0 12 0.0000 4 135 90 975 1500 1\001
4 0 0 50 0 0 12 0.0000 4 135 90 2250 1575 2\001
4 0 0 50 0 0 12 0.0000 4 135 90 2250 2400 3\001
4 0 0 50 0 0 12 0.0000 4 135 90 900 2475 4\001
4 0 0 50 0 0 12 0.0000 4 135 90 3075 1575 1\001
4 0 0 50 0 0 12 0.0000 4 135 90 4425 1575 2\001
4 0 0 50 0 0 12 0.0000 4 135 90 3000 2475 4\001
4 0 0 50 0 0 12 0.0000 4 135 90 4350 2400 3\001
4 0 0 50 0 0 20 0.0000 4 240 315 1425 900 [1]\001
4 0 0 50 0 0 12 0.0000 4 180 390 5775 1125 Edge\001
4 0 0 50 0 0 12 0.0000 4 135 420 6675 1125 Label\001
4 0 0 50 0 0 12 0.0000 4 135 90 6825 1425 0\001
4 0 0 50 0 0 12 0.0000 4 135 90 6825 1725 1\001
4 0 0 50 0 0 12 0.0000 4 135 90 6825 2025 2\001
4 0 0 50 0 0 20 0.0000 4 240 315 3600 900 [4]\001


==> figures/pansymm5hilbertbasis <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 1522 2122 75 75 1522 2122 1522 2197
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 2722 2122 75 75 2722 2122 2722 2197
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 2722 3322 75 75 2722 3322 2722 3397
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 1522 3322 75 75 1522 3322 1522 3397
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 2122 3922 75 75 2122 3922 2122 3997
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 4500 2100 75 75 4500 2100 4500 2175
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 5700 2100 75 75 5700 2100 5700 2175
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 4500 3300 75 75 4500 3300 4500 3375
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 5100 3900 75 75 5100 3900 5100 3975
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 5700 3300 75 75 5700 3300 5700 3375
1 2 2 1 0 7 50 0 -1 3.000 1 0.0000 4500 1800 150 225 4350 2025 4650 1575
1 2 2 1 0 7 50 0 -1 3.000 1 0.0000 5688 1862 150 225 5538 2087 5838 1637
1 2 2 1 0 7 50 0 -1 3.000 1 1.5708 5963 3301 150 225 6188 3451 5738 3151
1 2 2 1 0 7 50 0 -1 3.000 1 1.5708 4225 3313 150 225 4450 3463 4000 3163
1 1 0 1 0 7 50 0 -1 0.000 1 0.0000 2130 4189 150 225 2130 4189 1980 3964
1 1 0 1 0 7 50 0 -1 0.000 1 0.0000 1500 1879 150 225 1500 1879 1350 1654
1 1 0 1 0 7 50 0 -1 0.000 1 0.0000 2700 1879 150 225 2700 1879 2550 1654
1 2 0 3 0 7 50 0 -1 0.000 1 0.0000 5136 4128 150 225 4986 4353 5286 3903
1 1 0 1 0 7 50 0 -1 0.000 1 1.5708 1275 3300 150 225 1275 3300 1050 3450
1 1 0 1 0 7 50 0 -1 0.000 1 1.5708 2992 3304 150 225 2992 3304 2767 3454
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 6
	 1500 2100 1500 3300 2100 3900 2700 3300 2700 2100 1500 2100
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1500 2100 2700 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1500 3300 2700 2100
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1500 3300 2700 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1500 2175 2100 3900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2100 3900 2700 2100
2 1 0 3 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7500 3825 8100 3825
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 7500 3450 8100 3450
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 7500 3150 8100 3150
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 7200 2400 7200 4200 9300 4200 9300 2400 7200 2400
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 4500 2100 4500 3300 5700 3300 5700 2100 4500 2100
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 4500 2100 5100 3900
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 5100 3900 5700 2100
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 4575 2100 5700 3300
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 4500 3300 5700 2100
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 4500 3300 5100 3900
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 5100 3900 5700 3300
4 0 0 50 0 0 15 0.0000 4 150 105 1275 2250 1\001
4 0 0 50 0 0 15 0.0000 4 150 105 2925 2250 2\001
4 0 0 50 0 0 15 0.0000 4 150 105 2625 3600 3\001
4 0 0 50 0 0 15 0.0000 4 150 105 1425 3600 5\001
4 0 0 50 0 0 15 0.0000 4 150 105 1800 3975 4\001
4 0 0 50 0 0 15 0.0000 4 150 105 5925 2250 2\001
4 0 0 50 0 0 15 0.0000 4 150 105 4275 2250 1\001
4 0 0 50 0 0 15 0.0000 4 150 105 4800 3975 4\001
4 0 0 50 0 0 15 0.0000 4 150 105 5700 3600 3\001
4 0 0 50 0 0 15 0.0000 4 150 105 4425 3600 5\001
4 0 0 50 0 0 20 0.0000 4 240 315 4875 1500 [5]\001
4 0 0 50 0 0 20 0.0000 4 240 315 1800 1500 [1]\001
4 0 0 50 0 0 12 0.0000 4 180 390 7575 2925 Edge\001
4 0 0 50 0 0 12 0.0000 4 135 420 8475 2925 Label\001
4 0 0 50 0 0 12 0.0000 4 135 90 8475 3225 0\001
4 0 0 50 0 0 12 0.0000 4 135 90 8475 3525 1\001
4 0 0 50 0 0 12 0.0000 4 135 90 8475 3825 2\001


==> figures/pansymmhilbertbasis <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 2700 2700 75 75 2700 2700 2700 2775
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 1800 2700 75 75 1800 2700 1800 2775
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 2250 3600 75 75 2250 3600 2250 3675
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 1800 2700 2700 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2250 3600 1800 2700
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2250 3600 2700 2700
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 3675 3150 4275 3150
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 3375 2400 3375 3600 5250 3600 5250 2400 3375 2400
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 4
	 2250 3600 2400 3900 2100 3900 2250 3600
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 4
	 2730 2685 2580 2385 2880 2385 2730 2685
	 0.000 -1.000 -1.000 0.000
3 2 0 1 0 7 50 0 -1 0.000 0 0 0 4
	 1770 2640 1620 2340 1920 2340 1770 2640
	 0.000 -1.000 -1.000 0.000
4 0 0 50 0 0 12 0.0000 4 135 90 1575 2775 2\001
4 0 0 50 0 0 12 0.0000 4 135 90 2925 2775 3\001
4 0 0 50 0 0 12 0.0000 4 135 90 1950 3675 1\001
4 0 0 50 0 0 12 0.0000 4 180 390 3750 2925 Edge\001
4 0 0 50 0 0 12 0.0000 4 135 420 4575 2925 Label\001
4 0 0 50 0 0 12 0.0000 4 135 90 4725 3225 1\001
4 0 0 50 0 0 15 0.0000 4 195 255 2100 2325 [1]\001


==> figures/petersenhilbertbasis <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 1800 3600 75 75 1800 3600 1800 3675
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 2700 6600 75 75 2700 6600 2700 6675
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 225 4800 75 75 225 4800 225 4875
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 3310 4799 75 75 3310 4799 3310 4874
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 3300 7200 75 75 3300 7200 3300 7275
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 1800 3000 75 75 1800 3000 1800 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 -300 4800 75 75 -300 4800 -300 4875
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 300 7200 75 75 300 7200 300 7275
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 3900 4800 75 75 3900 4800 3900 4875
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 9622 7222 75 75 9622 7222 9622 7297
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 9000 6600 75 75 9000 6600 9000 6675
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 7200 6600 75 75 7200 6600 7200 6675
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 9600 4800 75 75 9600 4800 9600 4875
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 10200 4800 75 75 10200 4800 10200 4875
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 6525 4800 75 75 6525 4800 6525 4875
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 8100 3600 75 75 8100 3600 8100 3675
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 8100 3000 75 75 8100 3000 8100 3075
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 6000 4800 75 75 6000 4800 6000 4875
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 900 6600 75 75 900 6600 900 6675
1 3 0 1 0 7 50 0 0 0.000 1 0.0000 6600 7200 75 75 6600 7200 6600 7275
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 300 7200 900 6600
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2700 6600 3300 7200
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1800 3000 1800 3525
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3375 4800 3900 4800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 -300 4800 225 4800
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 6
	 8101 3622 7201 6622 9601 4822 6526 4822 9001 6622 8101 3622
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 6
	 1800 3000 -300 4800 300 7200 3300 7200 3900 4800 1800 3000
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 6
	 1800 3600 900 6600 3300 4800 225 4800 2775 6600 1800 3600
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 8100 3600 8100 3000
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 9600 4800 10200 4800
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 9000 6600 9600 7200
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 7200 6600 6600 7200
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 6450 4800 6000 4800
2 1 0 1 0 7 50 0 -1 3.000 0 0 -1 0 0 6
	 8100 3000 6000 4800 6600 7200 9600 7200 10200 4800 8100 3000
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 11400 5550 12000 5550
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 2
	 11400 5850 12000 5850
2 1 2 1 0 7 50 0 -1 3.000 0 0 -1 0 0 5
	 11100 5100 11100 6300 12900 6300 12900 5100 11100 5100
4 0 0 50 0 0 15 0.0000 4 150 105 8100 2850 1\001
4 0 0 50 0 0 15 0.0000 4 150 105 4050 4875 2\001
4 0 0 50 0 0 15 0.0000 4 150 105 3525 7275 3\001
4 0 0 50 0 0 15 0.0000 4 150 105 75 7275 4\001
4 0 0 50 0 0 15 0.0000 4 150 105 -525 4875 5\001
4 0 0 50 0 0 15 0.0000 4 150 105 1725 2775 1\001
4 0 0 50 0 0 15 0.0000 4 150 105 1950 3675 6\001
4 0 0 50 0 0 15 0.0000 4 150 105 675 6675 9\001
4 0 0 50 0 0 15 0.0000 4 150 105 2850 6675 8\001
4 0 0 50 0 0 15 0.0000 4 150 105 3300 5100 7\001
4 0 0 50 0 0 15 0.0000 4 150 210 150 5100 10\001
4 0 0 50 0 0 15 0.0000 4 150 105 8250 3675 6\001
4 0 0 50 0 0 15 0.0000 4 150 210 6450 5100 10\001
4 0 0 50 0 0 15 0.0000 4 150 105 5700 4875 5\001
4 0 0 50 0 0 15 0.0000 4 150 105 10350 4875 2\001
4 0 0 50 0 0 15 0.0000 4 150 105 6975 6675 9\001
4 0 0 50 0 0 15 0.0000 4 150 105 9150 6675 8\001
4 0 0 50 0 0 15 0.0000 4 150 105 9825 7275 3\001
4 0 0 50 0 0 15 0.0000 4 150 105 6375 7275 4\001
4 0 0 50 0 0 22 0.0000 4 195 285 8025 7650 P2\001
4 0 0 50 0 0 22 0.0000 4 195 285 1650 7650 P1\001
4 0 0 50 0 0 15 0.0000 4 150 105 9600 5100 7\001
4 0 0 50 0 0 12 0.0000 4 180 390 11475 5325 Edge\001
4 0 0 50 0 0 12 0.0000 4 135 90 12450 5625 1\001
4 0 0 50 0 0 12 0.0000 4 135 90 12450 5925 0\001
4 0 0 50 0 0 12 0.0000 4 135 420 12300 5325 Label\001
4 0 0 50 0 0 20 0.0000 4 240 315 7950 2400 [6]\001
4 0 0 50 0 0 20 0.0000 4 240 315 1650 2400 [6]\001

